Estimating and Improving Dynamic Treatment Regimes With a Time-Varying Instrumental Variable

Estimating dynamic treatment regimes (DTRs) from retrospective observational data is challenging as some degree of unmeasured confounding is often expected. In this work, we develop a framework of estimating properly defined "optimal" DTRs with a time-varying instrumental variable (IV) when unmeasured covariates confound the treatment and outcome, rendering the potential outcome distributions only partially identified. We derive a novel Bellman equation under partial identification, use it to define a generic class of estimands (termed IV-optimal DTRs), and study the associated estimation problem. We then extend the IV-optimality framework to tackle the policy improvement problem, delivering IV-improved DTRs that are guaranteed to perform no worse and potentially better than a pre-specified baseline DTR. Importantly, our IV-improvement framework opens up the possibility of strictly improving upon DTRs that are optimal under the no unmeasured confounding assumption (NUCA). We demonstrate via extensive simulations the superior performance of IV-optimal and IV-improved DTRs over the DTRs that are optimal only under the NUCA. In a real data example, we embed retrospective observational registry data into a natural, two-stage experiment with noncompliance using a time-varying IV and estimate useful IV-optimal DTRs that assign mothers to high-level or low-level neonatal intensive care units based on their prognostic variables.

==> old_tex/0203-review-framework.tex <==
%!TEX root = main.tex
\subsection{A General Framework of IV-Optimality}
\label{subsec:ITR general framework}
In this section, we present a general framework that incorporates the extra information in IVs for better policy estimation. 
This framwork is mathematically equivalent to the formulation in \eqref{eqn: middle ground of value interval} under certain conditions, but its conceptual simplicity makes it especially amenable when we shift our focus to (much more complicated) sequential deicision-making problems.

Conceptually, a valid IV and the associated identification assumptions impose \emph{distributional constraints} on potential outcome distributions $p^\star_a(\cdot|\bsx)$. For example, under assumptions leveraged in \cite{cui2019semiparametric} and \cite{qiu2020optimal}, $p^\star_a(\cdot|\bsx)$ can be expressed as functionals of the observed data distribution. 
As another example, if less stronger assumptions are imposed so that point identification is impossible, the partial identification results assert that $p^\star_a(\cdot|\bsx)$ is ``weakly bounded'', in the sense that for a sufficiently regular function $f$, we can find two functions $\underline{Q}(\bsx, a; f)$ and $\overline{Q}(\bsx, a; f)$ such that 
\begin{equation}
    \label{eq:weakly_boundedness}
    \underline{Q}(\bsx, a; f) \leq \int f(y) p^\star_a(dy|\bsx) \leq \overline{Q}(\bsx, a; f).
\end{equation}    
If $f$ is the identity function, then the above display is precisely the partial identification intervals of the mean conditional potential outcome $\bbE[Y(a)|\bsX=\bsx]$ that appeared in \eqref{eqn: middle ground of value interval}.
In both examples, a valid IV along with the identification assumptions allows us to specify a collection of distributions $\calP_{\bsx, a}$, so that 
$p^\star_a(\cdot|\bsx) \in \calP_{\bsx, a}$. In the first example, the set $\calP_{\bsx, a}$ is a singleton consisting of the ground truth potential outcome distribution $p^\star_a(\cdot|\bsx)$, whereas in the second example, the set $\calP_{\bsx, a}$ consists of all distributions that are weakly bounded in the sense of \eqref{eq:weakly_boundedness}. 
In words, $\calP_{\bsx, a}$ is the collection of all possible potential outcome distributions $p^\star_{a}(\cdot|\bsx)$ that are compatible with the putative IV and the associated IV identification assumptions, and we refer to it as an \emph{IV-constrained set}.
% instrumental variable puts constraints on the potential outcome distributions. Let $\calP_{\bsX, a}$, $a = \pm 1$, denote the collection of all possible potential outcome distributions $p^\ast_{a}(\cdot|\bsX)$ compatible with the putative IV $Z$ and the set of IV identification assumptions $\calC$. We will refer to $\calP_{\bsX, a}$ as the \emph{constraint sets}. Let $\calG_{\bsX, a} := \left\{\bbE_{p_{a}(\cdot|\bsX)}\left[Y(a)\right],~p_{a}(\cdot|\bsX) \in \calP_{\bsX, a}\right\}$ denote the collection of conditional average potential outcomes compatible with the constraint set $\calP_{\bsX, a}$, and we will refer to $\calG_{\bsX, a}$, $a = \pm1$, as the \emph{value sets}.

We may further equip an IV-constrained set $\calP_{\bsx, a}$ with a prior distribution $\scrP_{\bsx, a}$. Here, $\scrP_{\bsx,a}$ is a probability distribution on $\calP_{\bsx, a}$, the latter of which itself is a collection of probability distributions.  
For readers with a machine learning background, this is reminiscent of Baxter's model of inductive bias learning \citep{baxter2000model}: in his language, $\calP_{\bsx, a}$ is called an \emph{environment}, whose elements are called \emph{tasks}, and it is assumed that nature can sample a task from $\scrP_{\bsx, a}$, which is a probability distribution on the environment.
% denote probability measures on the constraint sets $\calP_{\bsX, a}$. 
To have a fully rigorous treatment, we equip $\calP_{\bsx, a}$ with a metric (e.g., Wasserstein metric) and work with the induced Borel sigma algebra (\citealp{parthasarathy2005probability}). 
% In the rest of the paper, we will not worry about measure-theoretic complications, as we will only invoke elementary properties of the expectation operator (e.g., Jensen's inequality). 

\begin{figure}[t!]
    \centering
    \begin{tikzpicture}[
squarednode/.style={rectangle, draw=red!60, fill=red!5, very thick}, 
every text node part/.style={align=center}
]
%Nodes
\node[squarednode] at (1,4) (IV) {Putative IV and \\ IV identification \\assumptions};
\node[squarednode] (constraint) [below=of IV] {Constraints on \\ $p^\star_{a}(\cdot|\bsx)$};
\node[squarednode] (P) [right=of constraint] {$\calP_{\bsx, a}$: collection of \\$p_{a}(\cdot |\bsx)$ compatible \\ with constraints};
\node[squarednode] (Estimand) [right=of P] {IV-constrained \\ value $V^\pi_{\scrP}$};
\node[squarednode] (Prior) [above=of Estimand]{$\scrP_{\bsx,a}$: prior \\ distributions \\ on $\calP_{\bsx, a}$};
\node[squarednode] (Estimator) [below=of Estimand] {IV-optimal \\ ITR};
%Lines
\draw[ultra thick, ->] (IV) -- (constraint);
\draw[ultra thick, ->] (constraint) -- (P);
\draw[ultra thick, ->] (P) -- (Estimand);
\draw[ultra thick, ->] (Estimand) -- (Estimator);
\draw[ultra thick, ->] (Prior) -- (Estimand);
\end{tikzpicture}
    \caption{\small A schematic plot of IV-optimality. A collection of prior distributions $\{\scrP_{\bsx, a}: \bsx\in \bbR^d, a = \pm 1\}$ is imposed on the IV-constrained sets $\{\calP_{\bsx, a}: \bsx\in \bbR^d, a = \pm 1\}$, which gives rise to the IV-constrained value $V^\pi_{\scrP}$. An ITR is IV-optimal with respect to this collection of priors if it maximizes $V^\pi_{\scrP}$ over a policy class $\Pi$.}
    \label{fig: scheme flowchat}
\end{figure}

Given the prior distributions $\{\scrP_{\bsx, a}: \bsx\in\calX, a =\pm 1\}$, we can define the \emph{IV-constrained value} of a policy $\pi$ as
% Associated with the constraint sets $\calP_{\bsX, a}$, the prior distributions $\scrP_{\textsf{prior},a}(\cdot|\bsX)$, and a policy $\pi(\cdot)$ is the following value function
\begin{equation}
  \label{eq:itr_general_estimand}
 V^\pi_{\scrP} = %\bbE[Y(\pi(\bsX))] = 
  \bbE_{\bsX}\bbE_{p_{\pi(\bsX)} \sim \scrP_{\bsX, \pi(\bsX)}}\bbE_{Y \sim p_{\pi(\bsX)}}[Y],
 % \bbE_{\bsX} \bigg[\bbE_{\scrP_{\textsf{prior}, a}(\cdot\mid\bsX)} \bbE_{p_{a}(\cdot|\bsX)}\left[Y(\pi(\bsX))\right]\bigg],
\end{equation}
where we write $p_{\pi(\bsx)} = p_{\pi(\bsx)}(\cdot|\bsx)$ for notational simplicity.
% The following definition extends the original notion of IV-optimality in \cite{pu2020estimating}.
% \begin{definition}
    % Let $\{\scrP_{\bsx, a}: \bsx\in\bbR^d, a =\pm 1\}$ a collection of prior distributions on the IV-constrained sets $\{\calP_{\bsx, a}: \bsx\in\bbR^d, a = \pm 1\}$. A policy is said to be IV-optimal with respect to 
% \end{definition}
From now on, we will refer to the collection of criteria given by maximizing $V^\pi_{\scrP}$ as \emph{IV-optimality}. 
An ITR is said to be \emph{IV-optimal} with respect to the prior distributions $\{\scrP_{\bsx, a}: \bsx\in\bbR^d, a =\pm 1\}$ and a policy class $\Pi$ if it maximizes $V^\pi_\scrP$ among all $\pi\in\Pi$. Flow chart in Figure \ref{fig: scheme flowchat} summarizes this conceptual framework.

It is clear that the formulation in \eqref{eqn: middle ground of value interval} can be recovered by carefully choosing the prior distributions. 
In particular, let $\underline{p}_a(\cdot|\bsx)$ and $\overline{p}_a(\cdot|\bsx)$ be distributions that witness the partial identification bounds $\underline{Q}(\bsx, a)$ and $\overline{Q}(\bsx, a)$, respectively:
\begin{equation}
    \label{eq:witness_ub_and_lb_single_stage}
\underline{Q}(\bsx, a) = \int y \underline{p}_a(dy|\bsx), \qquad \underline{Q}(\bsx, a) = \int y \overline{p}_a(dy|\bsx).
\end{equation}
Then the criterion \eqref{eqn: middle ground of value interval} can be recovered by considering the following two-point priors:
% Let $p_{\textsf{worst},a}(\cdot|\bsX) \in \calP_{\bsX, a}$ and $p_{\textsf{best},a}(\cdot|\bsX)\in \calP_{\bsX, a}$ denote the potential outcome distributions corresponding to $L_a(\bsX)$ and $U_a(\bsX)$, respectively. The estimand $V^{\textsf{mid}}(\pi; L_{\pm 1}, U_{\pm 1}, \alpha)$ is then equivalent to \eqref{eq:itr_general_estimand} with the following point mass prior distributions:
\begin{equation*}
    \scrP^{\textsf{two-point}}_{\bsx,a}
    =
    \lambda(\bsx, a)\cdot \delta_{\underline{p}_a(\cdot|\bsx)}
    + 
    [1-\lambda(\bsx, a)]\cdot \delta_{\overline{p}_a(\cdot|\bsx)},
    % \begin{cases}
    % p_{\textsf{worst},+1}(\cdot|\bsX),~\text{w.p.}~\alpha(\bsX),~\\
    % p_{\textsf{best},+1}(\cdot|\bsX),~\text{w.p.}~1 - \alpha(\bsX).
    % \end{cases}
    % \scrP^{\textsf{two-point}}_{\textsf{prior},-1}(\cdot|\bsX)=
    % \begin{cases}
    % p_{\textsf{worst},-1}(\cdot|\bsX),~\text{w.p.}~\alpha(\bsX),~\\
    % p_{\textsf{best},-1}(\cdot|\bsX),~\text{w.p.}~1 - \alpha(\bsX).
    % \end{cases}
\end{equation*}
where $\delta_p$ is a point mass at $p$.
As discussed near the end of Section \ref{subsec: IV optimality review}, setting $\lambda(\bsx, a)$ uniformly equal to $1/2$ recovers the original IV-optimality criterion considered in \citet{pu2020estimating} that minimizes the worst-case risk \eqref{eq:worst_case_risk_single_stage}. In fact, under certain regularity conditions, one can show that the reverse is also true: the formulation \eqref{eq:itr_general_estimand} for a specified collection prior distributions can also be recovered from \eqref{eqn: middle ground of value interval} by a careful choice of $\lambda$. 
In view of such an equivalence, the criterion \eqref{eq:itr_general_estimand} should \emph{not} be regarded as a generalization of \eqref{eqn: middle ground of value interval}. Rather, it is a convenient tool amenable to being generalized to the general multiple-stage setting. A proof of this equivalence statement will appear in Section \ref{sec: extension to DTR}. We defer how to estimate an IV-optimal ITR to Section \ref{sec: extension to DTR}.

% Further setting $\alpha(\bsX) = 1/2$ in $\scrP^{\textsf{two-point}}_{\textsf{prior},\pm 1}(\cdot \mid \bsX)$ restores the estimand that minimizes the worst-case misclassification error considered in \citet{pu2020estimating}.

% where $\bbE_{p_{a}(\cdot|\bsX)}[\cdot]$ denotes taking expectation of $Y(\pi(\bsX))$ with respect to the corresponding potential outcome distribution $p_{a}(\cdot|\bsX) \in \calP_{\bsX, a}$ and $\bbE_{\scrP_{\textsf{prior}, a}(\cdot\mid\bsX)}[\cdot]$ taking expectation of $p_{a}(\cdot|\bsX) \in \calP_{\bsX, a}$ with respect to $\scrP_{\textsf{prior}, a}(\cdot|\bsX)$. In the rest of this article, we will refer to the collection of criteria given by maximizing $V^\pi_{\textsf{IV}, \scrP_{\textsf{prior}}}$ as \emph{IV-optimality}. A policy is said to be \emph{IV-optimal} if it solves the optimization problem $\widehat{\pi} := \argmax_{\pi\in\calF}V^\pi_{\textsf{IV}, \scrP_{\textsf{prior}}}$. This framework slightly generalizes XX's framework and is amenable to generalization to a multiple-stage, dynamic treatment regime setting. Flow chart \ref{fig: scheme flowchat} summarizes the conceptual framework.


% One most popular class of IV partial identification results, e.g., Balke-Pearl bound, Manski-Pepper bound, etc, impose restrictions on potential outcome distributions $p^\ast_a(\cdot|\bsX)$ by bounding their first moments as follows:
% \begin{equation*}
% \label{eq:valid_distribution}
% p^\ast_a(\cdot|\bsX) \in \calP_{\bsX, a} = \left\{p_{a}(\cdot|\bsX): L_{a}(\bsX) \leq \int y p_{a}(y|\bsX) d\mu(y)\leq U_{a}(\bsX)\right\},~a = \pm1,
% \end{equation*}
% where $L_a(\bsx)$ and $U_a(\bsx)$ are bounding functions identified from observed data. The value sets $\calG_{\bsX, a}$ corresponding $\calP_{\bsX, a}$ are then immediately obtained in this case: $ \calG_{\bsX, a} = [L_a(\bsX), U_a(\bsX)]$, $a = \pm 1$.

% Let $p_{\textsf{worst},a}(\cdot|\bsX) \in \calP_{\bsX, a}$ and $p_{\textsf{best},a}(\cdot|\bsX)\in \calP_{\bsX, a}$ denote the potential outcome distributions corresponding to $L_a(\bsX)$ and $U_a(\bsX)$, respectively. The estimand $V^{\textsf{mid}}(\pi; L_{\pm 1}, U_{\pm 1}, \alpha)$ is then equivalent to \eqref{eq:itr_general_estimand} with the following point mass prior distributions:
% \begin{equation*}\scrP^{\textsf{two-point}}_{\textsf{prior},+1}(\cdot \mid \bsX)=
%     \begin{cases}
%     p_{\textsf{worst},+1}(\cdot|\bsX),~\text{w.p.}~\alpha(\bsX),~\\
%     p_{\textsf{best},+1}(\cdot|\bsX),~\text{w.p.}~1 - \alpha(\bsX).
%     \end{cases}
%     \scrP^{\textsf{two-point}}_{\textsf{prior},-1}(\cdot|\bsX)=
%     \begin{cases}
%     p_{\textsf{worst},-1}(\cdot|\bsX),~\text{w.p.}~\alpha(\bsX),~\\
%     p_{\textsf{best},-1}(\cdot|\bsX),~\text{w.p.}~1 - \alpha(\bsX).
%     \end{cases}
% \end{equation*}
% Further setting $\alpha(\bsX) = 1/2$ in $\scrP^{\textsf{two-point}}_{\textsf{prior},\pm 1}(\cdot \mid \bsX)$ restores the estimand that minimizes the worst-case misclassification error considered in \citet{pu2020estimating}.



==> old_tex/04-dtr.tex <==
%!TEX root = main.tex

\section{IV-Optimal Dynamic Treatment Regimes}
\label{sec: extension to DTR}

\subsection{Optimal and SRA-optimal Dynamic Treatment Regimes}
\label{subsec: DTR setup}
Consider a $K$-stage decision making problem as in \citet{murphy2003optimal} and \citet{schulte2014q}. At the first stage we are given baseline covariates $\bsX_1 = \bsx_1$, make a decision $a_1 = \pi_1(\bsx_1)$, and observe a reward $R_1(a_1) = r_1$. At stage $k$, $k = 2, \cdots, K$, let $\vec{a}_{k-1} = (a_1, \cdots, a_{k-1})$ denote treatment decisions from stage $1$ up to $k-1$, $\vec{R}_{k - 1}(\vec{a}_{k-1}) = (R_1(a_1), R_2(\vec{a}_2), \cdots, R_{k-1}(\vec{a}_{k-1}))$ rewards from stage $1$ to $k-1$, $\bsX_k(\vec{a}_{k - 1})$ new covariate information (e.g., time-varying covariates, auxiliary outcomes, etc) that would arise after stage $k-1$ but before stage $k$ if the patient were to follow the treatment decisions $\vec{a}_{k-1}$, and $\overline{\bsX}_k(\vec{a}_{k-1}) = (\bsX_1, \bsX_2(a_1), \cdots, \bsX_k(\vec{a}_{k-1}))$ the entire covariate history up to stage $k$. A possibly data-driven decision $a_k = \pi_k(\vec{a}_{k - 1}, \vec{r}_{k-1}, \overline{\bsx}_k)$ is then made and we observe reward $R_k$.
The goal is to estimate a dynamic treatment regime (or a policy) $\pi = (\pi_1, \pi_2, \cdots, \pi_K)$ such that the expected value of cumulative rewards $\sum_{k=1}^K r_k$ is maximized if the population were to follow the regime\footnote{In this paper, we focus on maximization of cumulative rewards. The generalization to maximizing $f(r_1, \cdots, r_K)$ for an arbitrary but known function $f$ is immediate.}. %In the rest of the article, we will always work with the cumulative rewards, i.e., $f(r_1, \cdots, r_K) = \sum_{k = 1}^K r_k$. }.
\sxc{Draw a diagram}

 
To simplify notations, at step $k$, the historical information available for making the $k$-th decision is denoted by
\begin{equation}
  \label{eq: hist_info}
  \vec{\bsH}_1 = \bsX_1,
  \qquad
  \vec\bsH_k = \big(\vec a_{k-1}, \vec R_{k-1}(\vec a_{k-1}), \vec\bsX_k(\vec a_{k-1})\big), ~ \forall 2\leq k \geq K.
\end{equation}
The information $\vec\bsH_k$ available at stage $k$ is composed of two parts, namely $\vec \bsH_{k-1}$ and $\bsH_k $, where $\vec\bsH_{k-1}$ is the information available at the previous stage and $\bsH_k = \big(a_{k-1}, R_{k-1}(\vec{a}_{k-1}), \bsX_k(\vec a_{k-1})\big)$ is the new information generated once decision $a_{k-1}$ has been made.
% $
  % \vec \bsH_k = (\vec \bsH_{k-1}, \bsH_k ), \bsH_k = \big(a_{k-1}, R_{k-1}(\vec{a}_{k-1}), \bsX_k(\vec a_{k-1})\big).
% $

Let $p^\star_{a_K}(\cdot|\vec\bsH_K)$ be the law of the reward at the final stage after decision $a_K$ has been made conditional on $\vec\bsH_K$:
\begin{equation}
  \label{eq: dtr_real_distr_K}
  \Big (R_K(\vec a_{K-1}, a_K)  ~|~ \vec\bsH_K\Big) \sim p^\star_{a_K}(\cdot|\vec\bsH_K).
\end{equation}
% with respect to the Lebesgue measure on $\bbR$. We note that generalizing to other dominating measures when the reward is not continuous is immediate.
For a regime $\pi = (\pi_1,\hdots, \pi_K)$, its \emph{action-value function} (or Q-function) and its \emph{value function} at stage $K$ can then be respectively defined as
\begin{align}
  \label{eq:true_Q_and_V_func_K}
  \Qfunc_K(\vec\bsH_K, a_K) & = \bbE^\star[R_K \mid \vec \bsH_K] = \bbE_{R_K \sim p^\star_{a_K}(\cdot |\vec\bsH_K)}[R_K],
  \qquad
  \Vfunc_K^\pi(\vec\bsH_K)  = Q_K^\pi\big( \vec\bsH_K, \pi_K(\vec\bsH_K) \big).
\end{align}
We emphasize that in the above display, the expectation operator $\bbE^\star[\cdot|\vec\bsH_K]$ is defined with respect to \eqref{eq: dtr_real_distr_K}: for a generic function $f(r)$, we have
$
  \bbE^\star[f(r) |\vec\bsH_{K}] =  \int f(r) \cdot p^\star_{a_K}(r|\vec\bsH_K) dr.
$
Meanwhile, note that the $Q$-function at stage $K$ has no dependence on $\pi$, whereas the corresponding value function depends on $\pi$ only through $\pi_K$.

With the foregoing notations, we are ready to define the $Q$-functions and the value functions at a generic stage $k\in[K]$ in a recursive fashion. In particular, for $k = K-1, \hdots, 1$, we let $p^\star_{a_k}(\cdot, \cdot | \vec\bsH_k)$ be the joint law of the immediate reward and the next-stage covariate after decision $a_k$ has been made conditional on $\vec\bsH_k$:
\begin{equation}
  \label{eq: dtr_real_distri_k}
  \Big( R_k(\vec{a}_{k-1}, a_k), \bsX_{k+1}(\vec{a}_{k-1}, a_k) ~|~ \vec\bsH_{k}\Big) \sim p^\star_{a_k}(\cdot, \cdot | \vec\bsH_k).
\end{equation}
For a regime $\pi$, we then define
\begin{align}
  \label{eq:true_Q_func_k}
  \Qfunc^\pi_k(\vec\bsH_k, a_k) & = \bbE^\star [R_k + \overbrace{\Vfunc^\pi_{k+1}(\vec\bsH_{k+1})}^{\textnormal{function of } (R_k, \bsX_{k+1})}  \mid {\vec\bsH_k}]= \bbE_{(R_k, \bsX_{k+1})\sim p^\star_{a_k}(\cdot, \cdot|\vec\bsH_k)}[R_k + \Vfunc^\pi_{k+1}(\vec\bsH_{k+1})]\\
  \label{eq:true_V_func_k}
  \Vfunc^\pi_k(\vec\bsH_k) & =  \Qfunc^\pi_k\big(\vec\bsH_k, \pi_k(\vec\bsH_k)\big).
\end{align}
Similar to \eqref{eq:true_Q_and_V_func_K}, the expectation operator $\bbE^\star[\cdot|\vec\bsH_k]$ is defined with respect to \eqref{eq: dtr_real_distri_k}: for a generic function $f(r, \bsx)$, we have
$
\bbE^\star[f(r, \bsx)|\vec\bsH_k] = \int f(r, \bsx) \cdot p^\star_{a_k}(r, \bsx|\vec\bsH_k) drd\bsx
$.
We interpret the $Q$-function $Q^\pi_k(\vec\bsH_k, a_k)$ as the cumulative rewards collected by executing $a_k$ at stage $k$ and follow $\pi$ from stage $k+1$ and onwards. In contrast, the value function $V^\pi_k(\vec\bsH_k)$ is the cumulative rewards collected by executing $\pi$ from stage $k$ and onwards.
Thus, $Q^\pi_k$ depends on $\pi$ only through $(\pi_{k+1},\hdots, \pi_K)$ and $V^\pi_k$ depends on $\pi$ only through $(\pi_k, \hdots, \pi_K)$.\footnote{For notational simplicity we interpret quantities whose subscripts do not make sense (e.g., $a_0, r_0$ and $\bsx_{K+1}$) as ``null'' quantities and their occurrences in mathematical expressions will be disregarded.}

A regime $\pi^\ast \in \mathcal{F}$ is said to be optimal if it maximizes $V^\pi_1(\bsx_1)$ for all fixed $\bsx_1$ (and hence $\bbE[V^\pi_1(\bsX_1)]$ for an arbitrary covariate distribution). To find an optimal regime, define the \emph{optimal value function} at stage $k$ as
\begin{equation}
\label{eq:opt_V_func_k}
\Vfunc^\star_k(\vec\bsH_k) = \max_{\pi_k, \hdots, \pi_K} \Vfunc^\pi_k(\vec\bsH_k),
\end{equation}
where the maximization is taken over all possible policies. A celebrated result from control theory states that the following \emph{dynamic programming} approach, also known as backward induction, yields an optimal regime $\pi^\ast$ (\citealp{murphy2003optimal, sutton2018reinforcement}):
\begin{align}
  \label{eq:opt_dtr_dynamic_prog_expression}
  \pi^\star_K(\vec\bsH_K) & = \argmax_{a_K\in\{\pm 1\}} \Qfunc_K(\vec\bsH_K, a_K), %, \\
  % \label{eq:opt_dtr_dynamic_prog_expression_K}
  ~~~~\pi^\star_k(\vec\bsH_k) = \argmax_{a_k\in\{\pm 1\}} \Qfunc^{\pi^\star}_k(\vec\bsH_k, a_k), ~~ k = K-1, \hdots, 1.
\end{align}
% \begin{enumerate}
    % \item At stage $K$, define
% \begin{equation}
  % \label{eq:opt_regime_K}
% $
  % \pi^\star_K(\vec\bsH_K) = \argmax_{a_K\in\{\pm 1\}} \Qfunc_K(\vec\bsH_K, a_K);
% $
% \end{equation}
% \item For $k = K-1, \hdots, 1$, recursively define
% \begin{equation}
  % \label{eq:opt_regime_k}
% $
%   \pi^\star_k(\vec\bsH_k) = \argmax_{a_k\in\{\pm 1\}} \Qfunc^{\pi^\star}_k(\vec\bsH_k, a_k).
% $
% \end{equation}
% \end{enumerate}
More explicitly, the regime $\pi^\ast$ defined above satisfies $\Vfunc^{\pi^\star}_k(\vec\bsH_k) = \Vfunc^\star(\vec\bsH_k)$ for any $k\in[K]$ and all configurations of $\vec\bsH_k$.

The foregoing discussion is based on the distributions imposed on the potential outcomes. To actually estimate the optimal regime, suppose we have collected i.i.d.~data from the law of the random trajectory $(\bsX_k^\obs, A_k^\obs, R_k^\obs)_1^K$, where we use the superscript $\obs$ to emphasize that they are the observations whose laws may or may not agree with the laws of the potential outcomes. We will sometimes drop the superscript $\obs$ when there is no ambiguity.
% The historical information $\vec{\bsH}^\obs_k$ available at stage $k$ is defined in a similar fashion to \eqref{eq: hist_info}.
Reminiscent of \eqref{eq: dtr_real_distr_K} and \eqref{eq: dtr_real_distri_k}, we let $p^\sra_{a_K}(\cdot | \vec\bsH_K), \{p^\sra_{a_k}(\cdot, \cdot|\vec\bsH_k)\}_{k=1}^{K-1}$ (with $\sra$ being the abbreviation of \emph{sequential randomization assumption}) be the laws of the observed rewards and covariates:
\begin{equation}
  \label{eq:dtr_obs_distr}
  \Big(R_k^\obs \mid \vec\bsH_K, A^\obs_K = a_K \Big) \sim p^\sra_{a_K}(\cdot |\vec\bsH_K ),
  ~~~~ \Big(R_k^\obs, \bsX_{k+1}^\obs \mid  \vec\bsH_k, A_k^\obs = a_k \Big) \sim p^\sra_{a_k}(\cdot, \cdot | \vec\bsH_k).
\end{equation}
Unlike $p^\ast_{a_k}(\cdot, \cdot \mid \vec\bsH_k)$, the law $p^\sra_{a_k}(\cdot, \cdot | \vec\bsH_k)$ is always identified from the observed data.
Let $\pi^\sra$ denote the regime obtained from the dynamic programming approach described below \eqref{eq:opt_V_func_k}, but using $p^\sra_{a_k}(\cdot, \cdot | \vec\bsH_k)$ in place of $p^\ast_{a_k}(\cdot, \cdot | \bsH_k)$. We will refer to $\pi^\sra$ as the \emph{SRA-optimal} DTR. Under a version of the sequential randomization assumptions and with addition assumptions of consistency and positivity, we have
$
  p^\star_{a_k}(\cdot, \cdot | \vec\bsH_k) = p^\sra_{a_k}(\cdot, \cdot | \vec\bsH_k),
$
from which it follows that $\pi^\sra = \pi^\star$, and thus is an optimal dynamic treatment regime (see, e.g., \citealt{schulte2014q}).

\subsection{The IV-optimal Estimand}
Suppose that in addition to the observed trajectories $(\bsX_k^\obs, A_k^\obs, R_k^\obs)_1^K$, we have access to a set of time-varying instrumental variables $\{Z_k\}_1^K$. Instrumental variables, along with the accompanying identification assumptions, imposes distributional constrains on the observed data. In particular, at stage $k$, one can construct from the data a collection of laws $\calP_{\vec\bsH_k, a_k}$, such that
\begin{equation}
p^\star_{a_k}(\cdot, \cdot | \vec\bsH_k)\in \calP_{\vec\bsH_k, a_k}.
\end{equation}
In words, the set $\calP_{\vec\bsH_k, a_k}$ is the collection of laws on the immediate reward and the next-stage covariate (after the decision $a_k$ has been made conditional on $\vec\bsH_k$) that are ``compatible'' with the IV identification assumptions.

Let $\scrP_{\vec\bsH_k, a_k}$ be a ``prior distribution'' on $\calP_{\vec\bsH_k, a_k}$. We use $p_{a_k}(\cdot,\cdot|\vec\bsH_k) \sim \scrP_{\vec\bsH_k, a_k}$ to denote that the law $p_{a_k}(\cdot, \cdot |\vec\bsH_k )\in \calP_{\vec\bsH_k, a_k}$ is sampled from the prior $\scrP_{\vec\bsH_k, a_k}$.
% and we write
% $$
  % p_{a_k}(\cdot,\cdot|\vec\bsH_k) \sim \scrP_{\vec\bsH_k, a_k}.
% $$
Note that $\scrP_{\vec\bsH_k, a_k}$ is a probability measure on a space of probability measures.  To have a fully rigorous treatment, we equip $\calP_{\vec\bsH_k, a_k}$ with a metric (e.g., Wasserstein metric) and work with its Borel sigma algebra.
In the rest of the paper, we will not worry about measure-theoretic complications, as we will only invoke elementary properties of the expectation operator (e.g., Jensen's inequality) \sxc{move to previous sections}.

At stage $K$, for fixed historical information $\vec\bsH_K$ and an action $a_K$, we define the \emph{IV-constrained $Q$-function} and the \emph{IV-constrained value function} of a regime $\pi$ with respect to the prior distribution $\scrP_{\vec\bsH_K, a_K}$ to be
\begin{align}
\label{eq:prior_Q_func_K}
\Qfunc_{\scrP, K}(\vec\bsH_K, a_K) & = \bbE_{\scrP}[R_K | \vec\bsH_K] = \bbE_{p_{a_K}(\cdot|\vec\bsH_K) \sim \scrP_{\vec\bsH_K, a_K}}\bbE_{R_K \sim p_{a_K}(\cdot|\vec\bsH_K)}[R_K]\\
\label{eq:prior_V_func_K}
\Vfunc_{\scrP, K}^\pi(\vec\bsH_K)  & = \Qfunc_{\scrP, K} \big(\vec\bsH_K,  \pi_K(\vec\bsH_K) \big)
\end{align}
respectively. Similar to \eqref{eq:true_Q_func_k} and \eqref{eq:true_V_func_k}, for $k = K-1, \hdots, 1$, we recursively define the IV-constrained $Q$ and value functions at stage $k$ as
\begin{align}
  \Qfunc^\pi_{\scrP, k}(\vec\bsH_k, a_k) & = \bbE_{\scrP}[R_k + {\Vfunc^\pi_{\scrP, k+1}(\vec\bsH_{k+1})}  \mid {\vec\bsH_k}] \nonumber\\
  \label{eq:prior_Q_func_k}
  & = \bbE_{p_{a_k}(\cdot,\cdot|\vec\bsH_k) \sim \scrP_{\vec\bsH_k, a_k}}\bbE_{(R_k, \bsX_{k+1})\sim p_{a_k}(\cdot, \cdot|\vec\bsH_k)}[R_k + \Vfunc^\pi_{\scrP, k+1}(\vec\bsH_{k+1})]\\
  \label{eq:prior_V_func_k}
  \Vfunc^\pi_{\scrP, k}(\vec\bsH_k) & =  \Qfunc^\pi_{\scrP, k}\big(\vec\bsH_k, \pi_k(\vec\bsH_k)\big).
\end{align}
Note that in \eqref{eq:prior_Q_func_K}--\eqref{eq:prior_V_func_k}, the expectation operator $\bbE_{\scrP}$ is defined via first sampling a distribution $p_{a_k}(\cdot, \cdot, |\vec\bsH_k)$ from the prior $\scrP_{\vec\bsH_k, a_k}$, and then sampling the pair of reward and the next-stage covariate from $p_{a_k}(\cdot, \cdot, |\vec\bsH_k)$.

With the aforementioned notations, we define the \emph{IV-optimal} dynamic treatment regime with respect to a collection of prior distributions $\{\scrP_{\vec\bsH_k, a_k}\}$ as any regime that solves the following optimization problem:
\begin{equation}
  \label{eq:iv_opt_dtr}
  \max_{\pi} \Vfunc^\pi_{\scrP, 1}(\bsx_1).
\end{equation}
In the above display, the objective function is defined with respect to a specific baseline covariate $\bsx_1$.
However, as the next proposition shows, the above optimization problem can be solved by a modified dynamic programming strategy (similar to \eqref{eq:opt_dtr_dynamic_prog_expression}), and the resulting IV-optimal DTR is independent of $\bsx_1$.

\begin{proposition}[Dynamic programming for IV-optimal DTR]
\label{prop:iv_opt_dtr_dynamic_prog}
Let $\pi^\star$ be recursively defined as follows:
\begin{align}
  \label{eq:iv_opt_dtr_dynamic_prog_expression}
  \pi^\star_K(\vec\bsH_K) & = \argmax_{a_K\in\{\pm 1\}} \Qfunc_{\scrP, K}(\vec\bsH_K, a_K), %\\
  % \label{eq:iv_opt_dtr_dynamic_prog_expression_k}
  ~~~~\pi^\star_k(\vec\bsH_k) = \argmax_{a_k\in\{\pm 1\}} \Qfunc^{\pi^\star}_{\scrP, k}(\vec\bsH_k, a_k), ~k = K-1, \hdots, 1.
\end{align}
% \begin{enumerate}
  % \item At stage $K$, define $\pi^\star_K(\vec\bsH_K) = \argmax_{a_K\in\{\pm 1\}} \Qfunc_{\scrP, K}(\vec\bsH_K, a_K)$;
  % \item For $k = K-1, \hdots, 1$, recursively define
  % $\pi^\star_k(\vec\bsH_k) = \argmax_{a_k\in\{\pm 1\}} \Qfunc^{\pi^\star}_{\scrP, k}(\vec\bsH_k, a_k)$.
% \end{enumerate}
Then the regime $\pi^\star$ satisfies
\begin{equation}
  \label{eq:iv_opt_dtr_k}
  V^{\pi^\star}_{\scrP, k}(\vec\bsH_k) = \max_{\pi} V^\pi_{\scrP, k}(\vec\bsH_k)
\end{equation}
for any stage $k$ and any configuration of the historical information $\vec\bsH_k$.
\end{proposition}
\begin{proof}
  We proceed by induction. At stage $K$, \eqref{eq:iv_opt_dtr_k} is true by construction. Suppose \eqref{eq:iv_opt_dtr_k} holds for any stage $t\geq k+1$ and any $\vec\bsH_t$. At stage $k$, we have
  \begin{align*}
    \Vfunc^{\pi^\star}_{\scrP,k}(\vec\bsH_k)
    & = \Qfunc_{\scrP,k}^{\pi^\star}\big(\vec\bsH_k, \pi^\star_{k}(\vec\bsH_k)\big) \\
    & = \max_{a_k\in\{\pm 1\}} \Qfunc_{\scrP,k}^{\pi^\star}\big(\vec\bsH_k, a_k\big)  \\
    & = \max_{a_k\in\{\pm 1\}}  \bbE_{p_{a_k}(\cdot,\cdot|\vec\bsH_k) \sim \scrP_{\vec\bsH_k, a_k}}\bbE_{(R_k, \bsX_{k+1})\sim p_{a_k}(\cdot, \cdot|\vec\bsH_k)}[R_k + \Vfunc^{\pi^\star}_{\scrP, k+1}(\vec\bsH_{k+1})] \\
    & \overset{(*)}{=} \max_{a_k\in\{\pm 1\}}  \bbE_{p_{a_k}(\cdot,\cdot|\vec\bsH_k) \sim \scrP_{\vec\bsH_k, a_k}}\bbE_{(R_k, \bsX_{k+1})\sim p_{a_k}(\cdot, \cdot|\vec\bsH_k)}[R_k + \max_{\pi}\Vfunc^{\pi}_{\scrP, k+1}(\vec\bsH_{k+1})] \\
    & \overset{(**)}{\geq} \max_{\substack{a_k\in\{\pm 1\} \\ \pi_{k+1}, \hdots, \pi_K}}
    \bbE_{p_{a_k}(\cdot,\cdot|\vec\bsH_k) \sim \scrP_{\vec\bsH_k, a_k}}\bbE_{(R_k, \bsX_{k+1})\sim p_{a_k}(\cdot, \cdot|\vec\bsH_k)}[R_k + \Vfunc^{\pi}_{\scrP, k+1}(\vec\bsH_{k+1})] \\
    & = \max_{\substack{a_k\in\{\pm 1\} \\ \pi_{k+1}, \hdots, \pi_K}} \Qfunc^{\pi}_{\scrP, k} (\vec\bsH_{k}, a_k)\\
    & = \max_{\pi_k, \hdots, \pi_K} \Vfunc_{\scrP,k}^\pi(\vec\bsH_k)
  \end{align*}
  where $(*)$ is by our inductive hypothesis and $(**)$ is by Jensen's inequality. Note that the reverse inequality $\Vfunc^{\pi^\star}_{\scrP,k}(\vec\bsH_k)  \leq \max_{\pi} \Vfunc_{\scrP,k}^\pi(\vec\bsH_k)$ holds by construction. Thus, the desired result follows.
\end{proof}





\subsection{Estimation of the IV-Optimal Dynamic Treatment Regime}
Estimating the IV-optimal DTR based on Proposition \ref{prop:iv_opt_dtr_dynamic_prog} alone is difficult, as the definitions of the $Q$ and value functions both involve integrating over the prior distributions $\{\scrP_{\vec\bsH_k, a_k}\}$. In this subsection, we provide a strategy for estimating the IV-optimal DTR that bypasses such an integration operation.

To start with, for a fixed history $\vec\bsH_K$ and an action $a_K$, we define the \emph{pessimistic and optimistic IV-constrained $Q$-functions} as well as the corresponding value functions for a regime $\pi$ as
\begin{align}
  \label{eq:worst_Q_and_V_func_K}
  \underline{\Qfunc}_{K}(\vec\bsH_K, a_K) & = \inf_{\substack{p_{a_K}(\cdot|\vec\bsH_K) \in \calP_{\vec\bsH_K, a_K} }} \bbE_{R_K\sim p_{a_K}(\cdot|\vec\bsH_K)} [R_K] ,
  ~~~~ \underline{\Vfunc}_K^\pi(\vec\bsH_K) = \underline{\Qfunc}_K\big(\vec\bsH_K, \pi_K(\vec\bsH_K)\big), \\
  \label{eq:best_Q_and_V_func_K}
  \overline{\Qfunc}_{K}(\vec\bsH_K, a_K) & = \sup_{\substack{p_{a_K}(\cdot|\vec\bsH_K) \in \calP_{\vec\bsH_K, a_K} }} \bbE_{R_K\sim p_{a_K}(\cdot|\vec\bsH_K)} [R_K] ,
  ~~~~ \overline{\Vfunc}_K^\pi(\vec\bsH_K) = \overline{\Qfunc}_K\big(\vec\bsH_K, \pi_K(\vec\bsH_K)\big).
  % \label{eq:best_rel_Q_func_K}
  % \overline{\Qfunc}_{K}^{\pi\rel\pibase}(\vec\bsH_K, a_K) & = \sup_{\substack{p_{a_K}(\cdot|\vec\bsH_K) \in \calP_{\vec\bsH_K, a_K} \\ p_{a'_{K}}(\cdot|\vec\bsH_K) \in \calP_{\vec\bsH_K, a_K'} }} \bigg\{ \bbE_{R_K\sim p_{a_K}(\cdot|\vec\bsH_K)} [R_K] - \bbE_{R_K'\sim p_{a'_K} (\cdot|\vec\bsH_K)}[R_K'] \bigg\},
\end{align}
% Analogously, the \emph{optimistic IV-constrained $Q$-function}, denoted as $\overline{\Qfunc}_K(\vec\bsH_K, a_K)$, and the corresponding value function, denoted as $\overline{\Vfunc}_K(\vec\bsH_K)$, are defined by replacing the $\inf$ symbol in the above two equations with the $\sup$ symbol, respectively.
Intuitively, the above two displays correspond to the ``worst case'' and the ``best case'' prior distributions, respectively.
% prior distribution that gives rise to the pessimistic (resp. optimistic) IV-constrained $Q$- and value functions, provided the infimum (resp. supremum) can be attained.
By construction, given arbitrary prior distributions $\scrP_{\vec\bsH_K, \pm 1}$, there exists some constants $\lambda(\vec\bsH_K, \pm 1)\in[0, 1]$ such that the resulting IV-constrained $Q$- and value function can be respectively written as
\begin{align}
  {\Qfunc}_{\scrP, K}(\vec\bsH_K, a_K) & = Q_{\lambda, K}(\vec\bsH_K, a_K) \nonumber\\
  \label{eq:wted_Q_func_K}
  & = \lambda(\vec\bsH_K, a_K) \cdot \underline\Qfunc_K(\vec\bsH_K, a_K) + \big(1 - \lambda(\vec\bsH_K, a_K) \big)\cdot \overline{\Qfunc}_K(\vec\bsH_K, a_K),\\
  % ~~~~ \underline{\Vfunc}_K^\pi(\vec\bsH_K) = \underline{\Qfunc}_K\big(\vec\bsH_K, \pi_K(\vec\bsH_K)\big).
  \label{eq:wted_V_func_K}
  \Vfunc_{\scrP, K}^\pi(\vec\bsH_K) & = \Vfunc_{\lambda, K}^\pi(\vec\bsH_K) = \Qfunc_{\lambda, K}\big(\vec\bsH_K, \pi_K(\vec\bsH_K)\big).
\end{align}

Now, for $k = K-1, \hdots, 1$, we recursively define the pessimistic and optimistic IV-constrained $Q$-functions as well as their weighted version as
\begin{align}
  \label{eq:worst_Q_func_k}
  \underline\Qfunc^\pi_{\lambda, k}(\vec\bsH_k, a_k) & = \inf_{p_{a_k} (\cdot,\cdot|\vec\bsH_k) \in \calP_{\vec\bsH_k, a_k}} \bbE_{(R_k, \bsX_{k+1})\sim p_{a_k}(\cdot, \cdot|\vec\bsH_k)}[R_k + \Vfunc^\pi_{\lambda, k+1}(\vec\bsH_{k+1})], \\
  \label{eq:best_Q_func_k}
  \overline\Qfunc^\pi_{\lambda, k}(\vec\bsH_k, a_k) & = \sup_{p_{a_k} (\cdot,\cdot|\vec\bsH_k) \in \calP_{\vec\bsH_k, a_k}} \bbE_{(R_k, \bsX_{k+1})\sim p_{a_k}(\cdot, \cdot|\vec\bsH_k)}[R_k + \Vfunc^\pi_{\lambda, k+1}(\vec\bsH_{k+1})],\\
  \label{eq:wted_Q_func_k}
  Q_{\lambda, k}^\pi(\vec\bsH_k, a_k)
  & = \lambda(\vec\bsH_k, a_k) \cdot \underline\Qfunc_{\lambda, k}^\pi(\vec\bsH_k, a_k) + \big(1 - \lambda(\vec\bsH_k, a_k) \big)\cdot \overline{\Qfunc}_{\lambda, k}^\pi(\vec\bsH_k, a_k).
\end{align}
The corresponding value functions, denoted defined as $\underline{\Vfunc}^\pi_{\lambda, k}, \overline\Vfunc^\pi_{\lambda, k}$, and $\Vfunc^\pi_{\lambda, k}$, are then defined by replacing $a_k$ in their $Q$-functions with $\pi_k(\vec\bsH_k)$.
Note carefully that the left-hand sides of \eqref{eq:worst_Q_func_k} and \eqref{eq:best_Q_func_k} are indexed by $\{\lambda(\vec\bsH_{t}, a_t)\}$ for $t\geq k+1$, whereas the left-hand side of \eqref{eq:wted_Q_func_k} is indexed by $\{\lambda(\vec\bsH_{t}, a_t)\}$ for $t\geq k$.
By a similar reasoning, for any prior distributions $\scrP_{\vec\bsH_k, \pm 1}$, one can choose $\lambda(\vec\bsH_k, \pm 1)$ to make the weighted $Q$-function $\Qfunc^\pi_{\lambda, k}$ (resp.~$\Vfunc^\pi_{\lambda, k}$) agree with the corresponding IV-constrained $Q$-function $\Qfunc^\pi_{\scrP, k}$ (resp.~$\Vfunc^\pi_{\scrP,k}$).

The foregoing discussion establishes that for any collection of prior distributions $\{\scrP_{\vec\bsH_k, a_k}\}$, there exists a collection of constants $\{\lambda(\vec\bsH_k, a_k)\}\subset [0, 1]$ such that the original IV-constrained $Q$-functions \eqref{eq:prior_Q_func_k} (resp.~value functions) agree with the convex combination of pessimistic and optimistic IV-constrained $Q$-functions \eqref{eq:wted_Q_func_k} (resp.~value functions).
If the reverse statement is also true, then we can deduce that specifying the priors $\{\scrP_{\vec\bsH_k, a_k}\}$ is equivalent to specifying the collection of constants $\{\lambda(\vec\bsH_k, a_k)\}$, in the sense that the collection of all IV-constrained $Q$- functions $\Qfunc^\pi_{\scrP, k}$'s (resp. $\Vfunc^\pi_{\scrP, k}$'s) as one varies the prior distributions is equal to the collection of all $\Qfunc^\pi_{\lambda, k}$'s (resp. $\Vfunc^\pi_{\lambda, k}$'s) as one varies the constants $\lambda(\vec\bsH_k, \pm 1)$.
Such an equivalence statement would then allow us to bypass the integration over the prior distributions by focusing on $\Qfunc^\pi_{\lambda, k}$ and $\Vfunc^\pi_{\lambda, k}$'s.

The following proposition asserts that this equivalence statement indeed holds under certain regularity conditions and gives a precise analytic expression for the IV-optimal DTR.

\begin{proposition}[Structure of the IV-optimal DTR]
\label{prop:struc_of_iv-opt_dtr}
Fix any collection of constants $\{\lambda(\vec\bsH_k, a_k)\}\subset [0, 1]$ and construct $\underline Q^\pi_{\lambda, k}, \overline Q^\pi_{\lambda, k}$ recursively as in \eqref{eq:worst_Q_and_V_func_K}--\eqref{eq:best_Q_and_V_func_K} and \eqref{eq:worst_Q_func_k}--\eqref{eq:best_Q_func_k}\footnote{For notational simplicity, we write $\underline{\Qfunc}_{K} = \underline{\Qfunc}_{\lambda, K}^\pi$ and $\overline{\Qfunc}_{K} = \overline{\Qfunc}_{\lambda, K}^\pi$, although they have no dependence on $\lambda$ and $\pi$. }.
Assume all the infimums and supremums in the definition of $\underline Q^\pi_{\lambda, k}$'s and $\overline Q^\pi_{\lambda, k}$'s can be attained.
Then, there exists a collection of prior distributions $\{\scrP_{\vec\bsH_k, a_k}\}$ such that
\begin{equation}
  \label{eq:equiv_iv_opt_dtr}
  \Qfunc^\pi_{\lambda, k} = \Qfunc^\pi_{\scrP, k}, \qquad \Vfunc^\pi_{\lambda, k} = \Vfunc^\pi_{\scrP, k}, ~~\forall k\in[K].
\end{equation}
Moreover, if we recursively define the regime $\pi^\star$ as
\begin{equation}
  \label{eq:struc_of_iv-opt_dtr}
  \pi^\star_k(\vec\bsH_k) = \sgn\big(L_{\lambda, k}^{\pi^\star}(\vec\bsH_k) +U_{\lambda, k}^{\pi^\star}(\vec\bsH_k) \big), ~~ k = K, \hdots, 1,
\end{equation}
where
\begin{align}
  \label{eq:lb_wted_cate}
  L_{\lambda, k}^{\pi}(\vec\bsH_k)
  & = \lambda(\vec\bsH_k, +1) \cdot \underline{\Qfunc}_{\lambda ,k}^{\pi} (\vec\bsH_k, +1) - \big(1-\lambda(\vec\bsH_k, -1)\big) \cdot \overline{\Qfunc}_{\lambda, k}^{\pi} (\vec\bsH_k, -1)\\
  \label{eq:lb_wted_cate}
  U_{\lambda, k}^{\pi}(\vec\bsH_k)
  & = \big(1-\lambda(\vec\bsH_k, +1)\big) \cdot \overline{\Qfunc}_{\lambda, k}^{\pi} (\vec\bsH_k, +1) - \lambda(\vec\bsH_k, -1) \cdot \underline{\Qfunc}_{\lambda,k}^{\pi} (\vec\bsH_k, -1)
\end{align}
then $\pi^\star$ is an IV-optimal DTR with respect to $\{\scrP_{\vec\bsH_k, a_k}\}$ in the sense of \eqref{eq:iv_opt_dtr_k}.
\end{proposition}
\begin{proof}
Equation \eqref{eq:struc_of_iv-opt_dtr} is proved by recursively constructing $\scrP_{\vec\bsH_k, a_k}$ be the two-point prior:
$$
  \scrP_{\vec\bsH_k, a_k} = \lambda(\vec\bsH_k, a_k) \cdot \delta_{\underline p_{a_K}(\cdot | \vec\bsH_k)} + \big(1 - \lambda(\vec\bsH_k, a_k)\big) \cdot \delta_{\overline p_{a_K}(\cdot | \vec\bsH_k)},
$$
where $\underline p_{a_K}(\cdot | \vec\bsH_k)$ and $\overline p_{a_K}(\cdot | \vec\bsH_k)$ are the distributions that attain the infimum and the supremum of \eqref{eq:worst_Q_func_k} and \eqref{eq:best_Q_func_k}, respectively. Given \eqref{eq:struc_of_iv-opt_dtr}, we invoke Proposition \ref{prop:iv_opt_dtr_dynamic_prog} to deduce that the IV-optimal DTR $\pi^\star$ can be recursively written as
\begin{align*}
  & \pi_k^\star(\vec\bsH_k) \\
  & = \argmax_{a_k \in\{\pm 1\}} \Qfunc^{\pi^\star}_{\scrP, k}(\vec\bsH_k, a_k) \\
  & = \argmax_{a_k\in\{\pm 1\}} \bigg\{\lambda(\vec\bsH_k, a_k) \cdot \underline\Qfunc_{\lambda, k}^{\pi^\star}(\vec\bsH_k, a_k) + \big(1 - \lambda(\vec\bsH_k, a_k) \big)\cdot \overline{\Qfunc}_{\lambda, k}^{\pi^\star}(\vec\bsH_k, a_k)\bigg\} \\
  & = \argmin_{a_k\in\{\pm 1\}} \bigg\{\indc{a_k = -1} \times
  \bigg[
  \lambda(\vec\bsH_k, +1) \cdot \underline \Qfunc^{\pi^\star}_{\lambda, k}(\vec\bsH_k, +1) + \big(1- \lambda(\vec\bsH_k, +1)\big) \cdot \overline\Qfunc^{\pi^\star}_{\lambda, k}(\vec\bsH_k, +1)  \\
  & \qquad\qquad\qquad\qquad\qquad\qquad - \lambda(\vec\bsH_k, -1) \cdot \underline \Qfunc^{\pi^\star}_{\lambda, k}(\vec\bsH_k, -1) + \big(1- \lambda(\vec\bsH_k, -1)\big) \cdot \overline\Qfunc^{\pi^\star}_{\lambda, k}(\vec\bsH_k, -1)
  \bigg]\bigg\} \\
  & = \argmin_{a_k\in\{\pm 1\}} \bigg\{\indc{a_k = -1} \times \bigg( L^{\pi^\star}_{\lambda, k}(\vec\bsH_k) + U^{\pi^\star}_{\lambda, k}(\vec\bsH_k) \bigg)\bigg\},
\end{align*}
from which \eqref{eq:struc_of_iv-opt_dtr} follows.
\end{proof}

Note that \eqref{eq:struc_of_iv-opt_dtr} is well-defined, as $L_{\lambda, k}^{\pi}(\vec\bsH_k)$ and $U_{\lambda, k}^{\pi}(\vec\bsH_k)$ depend on $\pi$ only through $\pi_{t}$ for $t\geq k+1$.
One can think of these two quantities as the effective lower and upper bounds on the conditional average treatment effect at stage $k$ when the regime $\pi$ is executed from stage $k+1$ and onwards. When $\lambda(\vec\bsH_k, a_K)$ is uniformly equal to $1/2$, then one readily checks that \eqref{eq:struc_of_iv-opt_dtr} can be equivalently expressed as follows:
$$
  \pi^\star(\vec\bsH_k) =
  \begin{cases}
    +1 & \textnormal{if } L_{\lambda, k}^{\pi^\star}(\vec\bsH_k) > 0 \\
    -1 & \textnormal{if } U_{\lambda, k}^{\pi^\star}(\vec\bsH_k) < 0 \\
    +1 & \textnormal{if } L_{\lambda, k}^{\pi^\star}(\vec\bsH_k) \leq 0\leq  U_{\lambda, k}^{\pi^\star}(\vec\bsH_k) \textnormal{ and } |U_{\lambda, k}^{\pi}(\vec\bsH_k)| \geq |L_{\lambda, k}^{\pi^\star}(\vec\bsH_k)| \\
    -1 & \textnormal{if } L_{\lambda, k}^{\pi^\star}(\vec\bsH_k) \leq 0\leq  U_{\lambda, k}^{\pi^\star}(\vec\bsH_k) \textnormal{ and } |U_{\lambda, k}^{\pi^\star}(\vec\bsH_k)| < |L_{\lambda, k}^{\pi^\star}(\vec\bsH_k)|.
  \end{cases}
$$
This has a simple interpretation as follows:
\begin{itemize}
  \item If $L_{\lambda, k}^{\pi^\star}(\vec\bsH_k) > 0$ or $U_{\lambda, k}^{\pi^\star}(\vec\bsH_k) < 0$, then we are certain about which action is better, so we simply execute that action;
  \item Otherwise, we decide the action according to the magnitudes of the upper and lower bounds.
  % If $L_{\lambda, k}^{\pi^\star}(\vec\bsH_k) \leq 0\leq  U_{\lambda, k}^{\pi^\star}(\vec\bsH_k)$, then
\end{itemize}

With some algebra, one can show that the regime defined in \eqref{eq:struc_of_iv-opt_dtr} is also the solution of the following optimization problem:
$$
  \pi^\star_k = \argmin_{\pi_k} \bigg|L_{\lambda, k}^{\pi^\star}(\vec\bsH_k) + U_{\lambda, k}^{\pi^\star}(\vec\bsH_k)\bigg| \cdot \Indc\bigg\{\sgn\bigg(L_{\lambda, k}^{\pi^\star}(\vec\bsH_k) + U_{\lambda, k}^{\pi^\star}(\vec\bsH_k)\bigg) \neq \pi_k(\vec\bsH_k)\bigg\}.
$$
Such a representation allows us to convert the original problem into recursively solving $K$ classification problems.


==> old_tex/0401-dtr.tex <==
%!TEX root = main.tex

\section{Estimating Dynamic Treatment Regimes with an Instrumental Variable}
\label{sec: extension to DTR}

% \subsection{Review: Optimal and SRA-Optimal Dynamic Treatment Regimes}
%\subsection{Estimation in the Absence of Unmeasured Confounding: Optimal and SRA-Optimal Policies}
\subsection{Optimal and SRA-Optimal DTRs}
\label{subsec: DTR setup}
We now consider a general $K$-stage decision making problem \citep{murphy2003optimal,schulte2014q}. 
At the first stage we are given baseline covariates $\bsX_1 = \bsx_1 \in \calX$, make a decision $a_1 = \pi_1(\bsx_1)$, and observe a reward $R_1(a_1) = r_1$. 
At stage $k = 2, \cdots, K$, let $\vec{a}_{k-1} = (a_1, \cdots, a_{k-1})$ denote treatment decisions from stage $1$ up to $k-1$. We also let $\vec{R}_{k - 1}(\vec{a}_{k-1}) = (R_1(a_1), R_2(\vec{a}_2), \cdots, R_{k-1}(\vec{a}_{k-1}))$ denote the rewards from stage $1$ to $k-1$. 
Meanwhile, denote by $\bsX_k(\vec{a}_{k - 1})$ new covariate information (e.g., time-varying covariates, auxiliary outcomes, etc) that would arise after stage $k-1$ but before stage $k$ if the patient were to follow the treatment decisions $\vec{a}_{k-1}$, and $\Vec{\bsX}_k(\vec{a}_{k-1}) = (\bsX_1, \bsX_2(a_1), \cdots, \bsX_k(\vec{a}_{k-1}))$ the entire covariate history up to stage $k$. 
Given the realizations of $\vec R_{r-1} = \vec r_{k-1}, \vec\bsX_{k} = \vec\bsx_k$,
a possibly data-driven decision $a_k = \pi_k(\vec{a}_{k - 1}, \vec{r}_{k-1}, \vec{\bsx}_k)$ is then made and we observe reward $R_k(\vec a_k) = r_k$. 
% \sxc{we need to mention somewhere that we will use policy to refer generically either an ITR or a DTR}
Our goal is to estimate a dynamic treatment regime $\pi = \{\pi_k\}_{k=1}^K$, such that the expected value of cumulative rewards $\sum_{k=1}^K r_k$ is maximized if the population were to follow $\pi$.
% \footnote{In this paper, we focus on maximization of cumulative rewards. The generalization to maximizing $f(r_1, \cdots, r_K)$ for an arbitrary but known function $f$ is immediate.}.

To simplify the notations, the historical information available for making the $k$-th decision at stage $k$ is denoted by
% \begin{equation}
  % \label{eq: hist_info}
  $
  \vec{\bsH}_1 = \bsX_1
  $
  for $k = 1$
  and 
  $
  \vec\bsH_k = \big(\vec a_{k-1}, \vec R_{k-1}(\vec a_{k-1}), \vec\bsX_k(\vec a_{k-1})\big)
  $  
  for any 
  $
  2\leq k \leq K.
  $
% \end{equation}
The information $\vec\bsH_k$ consists of $\vec \bsH_{k-1}$ and $\bsH_k $: $\vec\bsH_{k-1}$ is the information available at the previous stage and $\bsH_k = \big(a_{k-1}, R_{k-1}(\vec{a}_{k-1}), \bsX_k(\vec a_{k-1})\big)$ is the new information generated after decision $a_{k-1}$ is made. 
Let $p^\star_{a_K}(\cdot|\vec\bsh_K)$ be the conditional law of $R(\vec a_K)$ given a specific realization of the historical information $\vec\bsH_K = \vec\bsh_k$.
% \begin{equation}
%   \label{eq: dtr_real_distr_K}
%   \Big (R_K(\vec a_{K-1}, a_K)  ~|~ \vec\bsH_K\Big) \sim p^\star_{a_K}(\cdot|\vec\bsH_K).
% \end{equation}  
% with respect to the Lebesgue measure on $\bbR$. We note that generalizing to other dominating measures when the reward is not continuous is immediate. 
We define the \emph{action-value function} (or $Q$-function) at stage $K$ to be
% For a policy $\pi = (\pi_1,\hdots, \pi_K)$, its \emph{action-value function} (or Q-function) and \emph{value function} at stage $K$ are defined as 
\begin{equation}
  \label{eq:true_Q_stage_K}
  \Qfunc_K(\vec\bsh_K, a_K)  = \bbE[R_K(\vec a_K) \mid \vec \bsH_K=\vec\bsh_k] = \bbE_{R_K \sim p^\star_{a_K}(\cdot |\vec\bsh_K)}[R_K],
\end{equation}
where we emphasize that the expectation is taken over the potential outcome distribution $p^\star_{a_K}(\cdot|\vec\bsh_K)$.
For a policy $\pi$, its \emph{value function} at stage $K$ is then defined as 
\begin{equation}
  \label{eq:true_V_stage_K}
  % \Qfunc_K(\vec\bsH_K, a_K)  = \bbE[R_K(\vec a_K) \mid \vec \bsH_K] = \bbE_{R_K \sim p^\star_{a_K}(\cdot |\vec\bsH_K)}[R_K],
  \Vfunc_K^\pi(\vec\bsh_K)  = Q_K\big( \vec\bsh_K, \pi_K(\vec\bsh_K) \big),
\end{equation}
% \begin{align}
%   \label{eq:true_Q_and_V_func_K}
%   \Qfunc_K(\vec\bsH_K, a_K) & = \bbE^\star[R_K \mid \vec \bsH_K] = \bbE_{R_K \sim p^\star_{a_K}(\cdot |\vec\bsH_K)}[R_K], 
%   ~\text{and}~
%   \Vfunc_K^\pi(\vec\bsH_K)  = Q_K^\pi\big( \vec\bsH_K, \pi_K(\vec\bsH_K) \big),
% \end{align}
% respectively. We emphasize that in the above display, the expectation operator $\bbE^\star[\cdot|\vec\bsH_K]$ is defined with respect to \eqref{eq: dtr_real_distr_K}: for a generic function $f(r)$, we have
% $
%   \bbE^\star[f(r) |\vec\bsH_{K}] =  \int f(r) \cdot p^\star_{a_K}(r|\vec\bsH_K) dr.
% $
Note that the value function at stage $K$ depends on $\pi$ only through $\pi_K$.

Next, we define the $Q$-functions and the value functions at a generic stage $k\in[K]$ recursively (denote $[K] = \{1, \hdots, K\}$). In particular, for $k = K-1, \hdots, 1$, we let $p^\star_{a_k}(\cdot, \cdot | \vec\bsh_k)$ denote the joint law of the reward $R_k(\vec a_k)$ and new covariate information $\bsX_{k+1}(\vec a_k)$ observed immediately after decision $a_k$ has been made conditional on $\vec\bsH_k = \vec\bsh_k$.
% \begin{equation}
%   \label{eq: dtr_real_distri_k}
%   \Big( R_k(\vec{a}_{k-1}, a_k), \bsX_{k+1}(\vec{a}_{k-1}, a_k) ~|~ \vec\bsH_{k}\Big) \sim p^\star_{a_k}(\cdot, \cdot | \vec\bsH_k).
% \end{equation}  
The $Q$-function of $\pi$ at stage $k$ are then defined as: 
\begin{align}
  \Qfunc^\pi_k(\vec\bsh_k, a_k) & = \bbE [R_k(\vec a_k) + {\Vfunc^\pi_{k+1}(\vec\bsH_{k+1})}
  % ^{\textnormal{function of } (R_k, \bsX_{k+1})}  
  \mid {\vec\bsH_k = \vec\bsh_k}]\nonumber\\
  \label{eq:true_Q_func_k}
  & = \bbE_{(R_k, \bsX_{k+1})\sim p^\star_{a_k}(\cdot, \cdot|\vec\bsh_k)}[R_k + \Vfunc^\pi_{k+1}(\vec\bsH_{k+1})],
\end{align}
  % \label{eq:true_V_func_k}
% \end{align}
where $\vec \bsH_{k+1} = (\vec\bsh_k , a_{k}, R_{k}, \bsX_{k+1})$ is a function of $R_k$ and $\bsX_{k+1}$.
The corresponding value function of $\pi$ is taken to be 
$\Vfunc^\pi_k(\vec\bsh_k)  =  \Qfunc^\pi_k\big(\vec\bsh_k, \pi_k(\vec\bsh_k)\big).$
% \sxc{use $p^\star_{a_k}$, omit dependence on history when there is no ambiguity}
Similar to \eqref{eq:true_Q_stage_K}, the expectation is taken over the potential outcome distribution $p^\star_{a_k}(\cdot, \cdot|\vec\bsh_k)$. 
% defined with respect to \eqref{eq: dtr_real_distri_k}: for a generic function $f(r, \bsx)$, we have
% $
% \bbE^\star[f(r, \bsx)|\vec\bsH_k] = \int f(r, \bsx) \cdot p^\star_{a_k}(r, \bsx|\vec\bsH_k) drd\bsx 
% $.
We interpret the $Q$-function $Q^\pi_k(\vec\bsh_k, a_k)$ as the cumulative rewards collected by executing $a_k$ at stage $k$ and follow $\pi$ from stage $k+1$ and onwards. 
In contrast, the value function $V^\pi_k(\vec\bsh_k)$ is the cumulative rewards collected by executing $\pi$ from stage $k$ and onwards.
Therefore, $Q^\pi_k$ depends on $\pi$ only through $\pi_{(k+1):K} = (\pi_{k+1},\hdots, \pi_K)$ and $V^\pi_k$ depends on $\pi$ only through $\pi_{k:K}=(\pi_k, \hdots, \pi_K)$.\footnote{For notational simplicity we interpret quantities whose subscripts do not make sense (e.g., $a_0, r_0$ and $\bsx_{K+1}$) as ``null'' quantities and their occurrences in mathematical expressions will be disregarded.}

With a slight abuse of notation, we let $\Pi = \Pi_1\times \cdots \Pi_K$ be a policy class.
A DTR is said to be optimal with respect to $\Pi$ if it maximizes $V^\pi_1(\bsx_1)$ for all fixed $\bsx_1$ (and hence $\bbE[V^\pi_1(\bsX_1)]$ for an arbitrary covariate distribution) over the policy class $\Pi$. 

Assume for now that $\Pi$ consists of all DTRs (i.e., each $\Pi_k$ consists of all Boolean functions). 
% To find an optimal policy, define the \emph{optimal value function} at stage $k$ as
% \begin{equation}
% \label{eq:opt_V_func_k}
% \Vfunc^\star_k(\vec\bsH_k) = \max_{\pi_k, \hdots, \pi_K} \Vfunc^\pi_k(\vec\bsH_k),
% \end{equation}
% where the maximization is taken over all possible policies. 
A celebrated result from control theory states that the \emph{dynamic programming} approach below, also known as \emph{backward induction}, yields an optimal DTR $\pi^\star$ (\citealp{murphy2003optimal, sutton2018reinforcement}):
\begin{align}
  \label{eq:opt_dtr_dynamic_prog_expression}
  \pi^\star_K(\vec\bsh_K) & = \argmax_{a_K\in\{\pm 1\}} \Qfunc_K(\vec\bsh_K, a_K), %, \\
  % \label{eq:opt_dtr_dynamic_prog_expression_K}
  ~~~~\pi^\star_k(\vec\bsh_k) = \argmax_{a_k\in\{\pm 1\}} \Qfunc^{\pi^\star}_k(\vec\bsh_k, a_k), ~~ k = K-1, \hdots, 1.
\end{align}
% \begin{enumerate}
    % \item At stage $K$, define
% \begin{equation}
  % \label{eq:opt_regime_K}
% $
  % \pi^\star_K(\vec\bsH_K) = \argmax_{a_K\in\{\pm 1\}} \Qfunc_K(\vec\bsH_K, a_K);
% $
% \end{equation}
% \item For $k = K-1, \hdots, 1$, recursively define
% \begin{equation}
  % \label{eq:opt_regime_k}
% $
%   \pi^\star_k(\vec\bsH_k) = \argmax_{a_k\in\{\pm 1\}} \Qfunc^{\pi^\star}_k(\vec\bsH_k, a_k).
% $
% \end{equation}
% \end{enumerate}
More explicitly, $\pi^\star$ satisfies $\Vfunc^{\pi^\star}_k(\vec\bsh_k) = \max_{\pi} \Vfunc^\pi_k(\vec\bsh_k)$ for any $k\in[K]$ and any configuration of the historical information $\vec\bsh_k$, and is always well-defined as $Q^{\pi^\star}_k$ depends on $\pi^\star$ only through $\pi^\star_{(k+1):K}$.

The foregoing discussion is based on the potential outcome distributions. Suppose that we have collected i.i.d.~data from the law of the random trajectory $(\bsX_k^\obs, A_k^\obs, R_k^\obs)_{k = 1}^K$, where the superscript $\obs$ emphasizes the retrospective nature of the data. 
% We will sometimes drop the superscript $\obs$ when there is no ambiguity.
% The historical information $\vec{\bsH}^\obs_k$ available at stage $k$ is defined in a similar fashion to \eqref{eq: hist_info}. 
% \textcolor{red}{May want to add obs to $H_k$ as well.}
%Reminiscent of \eqref{eq:true_Q_stage_K} and \eqref{eq:true_Q_func_k}
Let $p^\obs_{a_K}(\cdot | \vec\bsh_K), \{p^\obs_{a_k}(\cdot, \cdot|\vec\bsh_k)\}_{k=1}^{K-1}$ 
be the conditional laws of the observed rewards and new covariate information identified from the observed data: 
\begin{equation*}
  % \label{eq:dtr_obs_distr}
  (R_K^\obs \mid \vec\bsH_K^\obs=\vec\bsh_k, A^\obs_K = a_K ) \sim p^\obs_{a_K}(\cdot |\vec\bsh_K ), 
  ~~ (R_k^\obs, \bsX_{k+1}^\obs \mid  \vec\bsH_k^\obs = \vec\bsh_k, A_k^\obs = a_k ) \sim p^\obs_{a_k}(\cdot, \cdot | \vec\bsh_k),
\end{equation*}  
for $k\leq K-1$. Here, $\vec\bsH_k^\obs$ denotes the observed historical information observed up to stage $k$.
Suppose that we obtain a DTR using the dynamic programming approach described in \eqref{eq:opt_dtr_dynamic_prog_expression} with $p^\obs_{a_k}$ in place of $p^\star_{a_k}$.
Under a version of the sequential randomization assumptions (\citealp{robins1998marginal}) and with additional assumptions of consistency and positivity, we have
$
  p^\star_{a_k} = p^\obs_{a_k},
$
from which it follows that the DTR obtained is in fact an optimal DTR \citep{murphy2003optimal, schulte2014q}.
In view of this fact, we will refer to this policy as an \emph{SRA-optimal} DTR and denote it as $\pi^\sra$. Methods that estimate SRA-optimal DTRs have been well studied in the literature. See \cite{murphy2003optimal, zhao2015new,tao2018tree,zhang2018c}, among others.



\subsection{IV-Optimality for DTRs and Dynamic Programming Under Partial Identification}\label{subsec:IV Optimality DTR and bellman equation}

Suppose that in addition to the observed trajectory $(\bsX_k^\obs, A_k^\obs, R_k^\obs)_{k = 1}^K$, we have access to a time-varying instrumental variable $\{Z_k\}_{k = 1}^K$.
Similar to the single-stage setting in Section \ref{subsec:ITR general framework}, the IV, along with its associated identification assumptions, imposes distributional constraints on the potential outcome distributions $p^\star_{a_k}(\cdot, \cdot|\vec\bsh_k)$. 
That is, we can specify, for each action $a_k$ and historical information $\vec\bsh_k$ at stage $k$, an IV-constrained set $\calP_{\vec\bsh_k, a_k}$, which contains the ground truth potential outcome distribution $p^\star_{a_k}(\cdot, \cdot | \vec\bsh_k)$.
% $p^\star_{a_k}(\cdot, \cdot | \vec\bsH_k)\in \calP_{\vec\bsH_k, a_k}$.
Again, two primary examples are that $\calP_{\vec\bsh_k, a_k}$ is a singleton under point identification (\citealt{michael2020instrumental}), and that $\calP_{\vec\bsh_k, a_k}$ contains weakly bounded distributions by the partial identification intervals in the sense of \eqref{eq:weakly_boundedness}. For ease of exposition, we treat $\calP_{\vec\bsh_k, a_k}$ as a generic set of distributions compatible with the IV and identification assumptions for now; examples of $\calP_{\vec\bsh_k, a_k}$ will be given in Section \ref{subsec: estimate IV-optimal DTR} when we formally describe estimation procedures.
 
It is essential to have a time-varying IV (e.g., daily precipitation) rather than a time-independent IV (e.g., sickle cell trait) in the multiple-stage setting; see Supplementary Materials \textcolor{red}{X} for details.
 
Given the IV-constrained set $\calP_{\vec\bsh_k, a_k}$, we can impose a prior distribution $\scrP_{\vec\bsh_k, a_k}$ on it. This notion is, of course, a generalization of what was introduced in the single-stage setting in Section \ref{subsec:ITR general framework}.
We use $p_{a_k}(\cdot,\cdot|\vec\bsh_k) \sim \scrP_{\vec\bsh_k, a_k}$ to denote sampling a distribution $p_{a_k}(\cdot, \cdot |\vec\bsh_k )\in \calP_{\vec\bsh_k, a_k}$ from $\scrP_{\vec\bsh_k, a_k}$. 
% Notations here generalize those introduced in the single-stage setting in Section \ref{subsec:ITR general framework}. 
We will use the shorthand $p_{a_k}$ for $p_{a_k}(\cdot,\cdot|\vec\bsh_k)$ where there is no ambiguity.

Under the current notations, analogous to the conventional $Q$- and value functions defined in \eqref{eq:true_Q_stage_K}--\eqref{eq:true_Q_func_k}, we introduce their \emph{IV-constrained} counterparts.

\begin{definition}[IV-constrained $Q$- and value function]\label{def:DTR IV-constrained Q and value function}
% Let $\vec\bsH_k$ denote historical information and $a_k$ an action at stage $k$ for $k \in [K]$. 
For each stage $k\in[K]$, each action $a_k\in\{\pm 1\}$, and each configuration the historical information $\vec\bsH_k$, let $\scrP_{\vec\bsh_k, a_k}$ be a prior distribution on the IV-constrained set $\calP_{\vec\bsh_k, a_k}$. 
The IV-constrained $Q$-function and the corresponding value function of a DTR $\pi$ with respect to the collection prior distributions $\{\scrP_{\vec\bsh_k, a_k}\}$ at stage $K$ are
\begin{align}
\label{eq:prior_Q_func_K}
\Qfunc_{\scrP, K}(\vec\bsh_K, a_K) %= \bbE_{\scrP}[R_K | \vec\bsH_K] 
&= \bbE_{p_{a_K} \sim \scrP_{\vec\bsh_K, a_K}}\bbE_{R_K \sim p_{a_K}}[R_K],\\
\label{eq:prior_V_func_K}
\text{and}\qquad\Vfunc_{\scrP, K}^\pi(\vec\bsh_K) &= \Qfunc_{\scrP, K} \big(\vec\bsh_K,  \pi_K(\vec\bsh_K) \big),
\end{align}
respectively. 
Recursively, at stage $k = K - 1, K - 2, \cdots, 1$, the IV-constrained $Q$-function and the corresponding value function are
\begin{align}
  \Qfunc^\pi_{\scrP, k}(\vec\bsh_k, a_k) %&= \bbE_{\scrP}[R_k + {\Vfunc^\pi_{\scrP, k+1}(\vec\bsH_{k+1})}  \mid {\vec\bsH_k}] \nonumber\\
  \label{eq:prior_Q_func_k}
   &= 
   \bbE_{p_{a_k} \sim \scrP_{\vec\bsh_k, a_k}}\bbE_{(R_k, \bsX_{k+1})\sim p_{a_k}}[R_k + \Vfunc^\pi_{\scrP, k+1}(\vec\bsH_{k+1})],\\
  \label{eq:prior_V_func_k}
  \text{and}\qquad\Vfunc^\pi_{\scrP, k}(\vec\bsh_k) &=  \Qfunc^\pi_{\scrP, k}\big(\vec\bsh_k, \pi_k(\vec\bsh_k)\big),
\end{align}
respectively, where we recall that $\vec \bsH_{k+1} = (\vec\bsh_k , a_{k}, R_{k}, \bsX_{k+1})$ is a function of $R_k$ and $\bsX_{k+1}$.
\end{definition}

% \sxc{given the space we have probably we don't need to introduce $\bbE_{\scrP}$}
% In Definition \ref{def:DTR IV-constrained Q and value function}, the expectation operator $\bbE_{\scrP}[\cdot]$ is a shorthand for first sampling a distribution $p_{a_k}$ from $\scrP_{\vec\bsH_k, a_k}$ and then sampling the reward $R_k$ and new covariate information $\bsX_{k+1}$ from $p_{a_k}$. 
Definition \ref{def:DTR IV-constrained Q and value function} generalizes the notion of IV-constrained value in the single-stage setting.
Similar to the conventional $Q$- and value functions, the IV-constrained $Q$-function $Q^\pi_{\scrP,k}$ depends on $\pi$ only through $\pi_{(k+1):K}$ and the IV-constrained value function $V^\pi_{\scrP, k}$ depends on $\pi$ only through $\pi_{k:K}$.

Definition \ref{def:IV-Optimal DTR} follows from Definition \ref{def:DTR IV-constrained Q and value function} and defines the notion of IV-optimality for DTRs.

\begin{definition}[IV-optimal DTR]\label{def:IV-Optimal DTR}
% Let $\{Z_k\}_{k = 1}^K$ be a time-varying instrumental variable, $\big\{\calP_{\vec\bsH_k, a_k},~k\in[K]\big\}$ constraint sets, $\big\{\scrP_{\vec\bsH_k, a_k},~k\in[K]\big\}$ prior distributions on constraint sets, $\bsx_1$ baseline covariates at stage $1$, and $\Vfunc^\pi_{\scrP, 1}(\bsx_1)$ the IV-constrained value function at stage $1$ as defined in Definition \ref{def:DTR IV-constrained Q and value function}. 
% 
A DTR $\pi^\star$ is said to be IV-optimal with respect to the collection of prior distributions $\{\scrP_{\vec\bsh_k, a_k}\}$ and a policy class $\Pi$ if it satisfies 
% A dynamic treatment regime $\pi^\star$ is said to be IV-optimal if for any $\bsx_1\in\calX$, it satisifes
\begin{equation}
  \label{eq:iv_opt_dtr}
  \pi^\star \in \argmax_{\pi\in\Pi} \Vfunc^\pi_{\scrP, 1}(\bsx_1)
\end{equation}
for every fixed $\bsh_1 = \bsx_1\in\calX$.
\end{definition}

Note that a priori, we do not know if an IV-optimal policy $\pi^\star$ exists, as the above definition requires $\pi^\star$ to maximize the IV-constrained value function for every fixed $\bsx_1$ (and thus $\bbE_{\bsX_1}[V^\pi_{\scrP, 1}(\bsX_1)]$ for any law of $\bsX_1$). However, as we will see in our first main result below, the optimization problem \eqref{eq:iv_opt_dtr} can be solved via a modified dynamic programming algorithm if $\Pi$ consists of all policies.

\begin{theorem}[Dynamic programming for the IV-optimal DTR]
\label{thm:iv_opt_dtr_dynamic_prog}
Let $\pi^\star$ be recursively defined as follows:
\begin{align}
  \label{eq:iv_opt_dtr_dynamic_prog_expression}
  \pi^\star_K(\vec\bsh_K) & = \argmax_{a_K\in\{\pm 1\}} \Qfunc_{\scrP, K}(\vec\bsh_K, a_K), %\\
  % \label{eq:iv_opt_dtr_dynamic_prog_expression_k}
  ~~~~\pi^\star_k(\vec\bsh_k) = \argmax_{a_k\in\{\pm 1\}} \Qfunc^{\pi^\star}_{\scrP, k}(\vec\bsh_k, a_k), ~k \leq K-1.
\end{align}
% \begin{enumerate}
  % \item At stage $K$, define $\pi^\star_K(\vec\bsH_K) = \argmax_{a_K\in\{\pm 1\}} \Qfunc_{\scrP, K}(\vec\bsH_K, a_K)$;
  % \item For $k = K-1, \hdots, 1$, recursively define
  % $\pi^\star_k(\vec\bsH_k) = \argmax_{a_k\in\{\pm 1\}} \Qfunc^{\pi^\star}_{\scrP, k}(\vec\bsH_k, a_k)$.
% \end{enumerate}
Then the DTR $\pi^\star$ satisfies
\begin{equation}
  \label{eq:iv_opt_dtr_k}
  V^{\pi^\star}_{\scrP, k}(\vec\bsh_k) = \max_{\pi} V^\pi_{\scrP, k}(\vec\bsh_k)
\end{equation}
for any stage $k$ and any configuration of the historical information $\vec\bsh_k$, where the maximization is taken over all DTRs.
\end{theorem}

The above result is a generalization of the classical dynamic programming algorithm \eqref{eq:opt_dtr_dynamic_prog_expression} under partial identification. Note that the policy $\pi^\star$ appeared in the above theorem is always well-defined as $\Qfunc^{\pi^\star}_{\scrP_k}$ depends on $\pi^\star$ only through $\pi^\star_{(k+1):K}$.

\subsection{An Alternative Characterization of IV-Optimal DTRs} 
\label{subsec:alternative characterization}
% and A \texorpdfstring{$Q$}{Q}-Learning Algorithm}
Estimating an IV-optimal DTR based on Theorem \ref{thm:iv_opt_dtr_dynamic_prog} alone is difficult, primarily because the definitions of the IV-constrained $Q$- and value functions involve integration over the prior distributions $\{\scrP_{\vec\bsh_k, a_k}\}$. 
In this subsection, we provide an alternative characterization of an IV-optimal DTR which illuminates a practical estimation strategy. 

Recall that in the single-stage setting, there is an equivalence between the IV constrained value \eqref{eq:itr_general_estimand} and the convex combination of the lower and upper bounds of the value \eqref{eqn: middle ground of value interval}. The latter expression \eqref{eqn: middle ground of value interval} is easier to compute as long as the weights of the convex combination are specified. Below, we extend such an equivalence relationship to the multiple-stage setting and use it to get rid of the intractable integration over prior distributions. 

We start by defining the \emph{worst-case} and \emph{best-case} IV-constrained $Q$- and value functions as well as their weighted versions as follows.
% $\pi$.
% \sxc{I changed $\vec\bslam$ to $\vec\lambda$ as we have been using VEC to denote temporal vectors and bold symbol, like $\bsx$, to denote vectors that are multi-dimensional even without any temporal structure.}

\begin{definition}[Worst-case, best-case, and weighted $Q$- and value functions]\label{def:worst/best Q and value function}
Let the prior distributions $\{\scrP_{\vec\bsh_k, a_k}\}$ be specified and let $\{\lambda_k(\vec\bsH_k, a_k)\}$ be a collection of weighting functions taking values in $[0, 1]$.
The worst-case, best-case, and weighted $Q$-functions at stage $K$ with respect to the specified prior distributions and weighting functions are respectively defined as
\begin{align}
  \label{eq:worst Q stage K}
  &\underline{\Qfunc}_{K}(\vec\bsh_K, a_K) = \inf_{\substack{p_{a_K}\in \calP_{\vec\bsh_K, a_K}}} \bbE_{R_K\sim p_{a_K}} [R_K] , \\
  \label{eq:best Q stage K}
  &\overline{\Qfunc}_{K}(\vec\bsh_K, a_K) = \sup_{\substack{p_{a_K} \in \calP_{\vec\bsh_K, a_K} }} \bbE_{R_K\sim p_{a_K}} [R_K], \\
  \label{eq:wted_Q_func_K}
  &Q_{\vec{{\lambda}}, K}(\vec\bsh_K, a_K) = \lambda_K(\vec\bsh_K, a_K) \cdot \underline\Qfunc_K(\vec\bsh_K, a_K) + \big(1 - \lambda_K(\vec\bsh_K, a_K) \big)\cdot \overline{\Qfunc}_K(\vec\bsh_K, a_K),
\end{align}
% For a function $\lambda_K(\vec\bsH_K, \pm 1)\in [0, 1]$, the weighted $Q$-function at stage $K$ is
% \begin{equation}
% \label{eq:wted_Q_func_K}
  % Q_{\vec{{\lambda}}, K}(\vec\bsH_K, a_K) = \lambda_K(\vec\bsH_K, a_K) \cdot \underline\Qfunc_K(\vec\bsH_K, a_K) + \big(1 - \lambda_K(\vec\bsH_K, a_K) \big)\cdot \overline{\Qfunc}_K(\vec\bsH_K, a_K).
% \end{equation}
% where $\lambda_K(\vec\bsH_K, \pm 1)\in [0, 1]$ are some constants between $0$ and $1$. 
The corresponding worst-case, best case, and weighted value functions, denoted as $\underline{\Vfunc}_K^\pi(\vec\bsh_K)$, $\overline{\Vfunc}_K^\pi(\vec\bsh_K)$, and $\Vfunc_{\vec{{\lambda}}, K}^\pi(\vec\bsh_K)$ respectively, for a DTR $\pi$ are
% , and $\Vfunc_{\vec{{\lambda}}, K}^\pi(\vec\bsH_K)$ are 
obtained by setting $a_k = \pi_K(\vec\bsh_K)$ in the above displays. 
Recursively, at stage $k = K - 1, \cdots, 1$, we define the worst-case, best-case, and weighted Q-functions as
\begin{align}
  \label{eq:worst_Q_func_k}
  \underline\Qfunc^\pi_{\vec{\lambda}, k}(\vec\bsh_k, a_k) & = \inf_{p_{a_k} \in \calP_{\vec\bsh_k, a_k}} \bbE_{(R_k, \bsX_{k+1})\sim p_{a_k}}[R_k + \Vfunc^\pi_{\vec{\lambda}, k+1}(\vec\bsH_{k+1})], \\
  \label{eq:best_Q_func_k}
  \overline\Qfunc^\pi_{\vec{\lambda}, k}(\vec\bsh_k, a_k) & = \sup_{p_{a_k}\in \calP_{\vec\bsh_k, a_k}} \bbE_{(R_k, \bsX_{k+1})\sim p_{a_k}}[R_k + \Vfunc^\pi_{\vec{\lambda}, k+1}(\vec\bsH_{k+1})],\\
  \label{eq:wted_Q_func_k}
  Q_{\vec{\lambda}, k}^\pi(\vec\bsh_k, a_k) 
  & = \lambda_k(\vec\bsh_k, a_k) \cdot \underline\Qfunc_{\vec{\lambda}, k}^\pi(\vec\bsh_k, a_k) + \big(1 - \lambda_k(\vec\bsh_k, a_k) \big)\cdot \overline{\Qfunc}_{\vec{\lambda}, k}^\pi(\vec\bsh_k, a_k),
\end{align}
respectively.
% where $\lambda(\vec\bsH_k, \pm 1) \in [0, 1]$ are some constants between $0$ and $1$. 
Again, replacing $a_k$ in the above Q-functions with $\pi_k(\vec\bsh_k)$ yields their corresponding value functions $\underline{\Vfunc}^\pi_{\vec{\lambda}, k}, \overline\Vfunc^\pi_{\vec{\lambda}, k}$, and $\Vfunc^\pi_{\vec{\lambda}, k}$.
\end{definition}

Definition \ref{def:worst/best Q and value function} generalizes the criterion \eqref{eqn: middle ground of value interval}. According to Definition \ref{def:worst/best Q and value function}, the worst-case and best-case $Q$-functions $\underline\Qfunc^\pi_{\vec{\lambda}, k}$ and $\overline\Qfunc^\pi_{\vec{\lambda}, k}$ depend on the weighting functions only through $\lambda_t(\vec\bsh_{t}, a_t)$ for $k+1 \leq t \leq K\}$, whereas the corresponding value functions depend on the weighting functions only through $\lambda_t(\vec\bsh_{t}, a_t)$ for $k \leq t \leq K$. 
For notational simplicity, in the rest of the paper, we add superscript $\pi$ and subscript $\vec\lambda$ in $Q$-functions at stage $K$ (e.g., we write $\underline{Q}_K = Q^\pi_{\vec\lambda, K}$), although they have no dependence on $\pi$ and the weighting functions.

Theorem \ref{thm:struc_of_iv-opt_dtr} below establishes the equivalence between the weighted $Q$-functions (resp.~value functions) and their IV-constrained counterparts in Definition \ref{def:DTR IV-constrained Q and value function}.

\begin{theorem}[Equivalence between weighted and IV-constrained $Q$- and value functions]
%Alternative Characterization and Construction of IV-Optimal DTR]
\label{thm:struc_of_iv-opt_dtr}
The following two statements hold:
\begin{enumerate}
  \item Fix any collection of weighting functions $\{\lambda_k(\vec\bsh_k, a_k)\}$. Assume that in Definition \ref{def:worst/best Q and value function}, the infimums and supremums when defining weighted $Q$- and value functions are all attained. 
  Then there exists a collection of prior distributions $\{\scrP_{\vec\bsh_k, a_k}\}$ such that
  \begin{equation}
  \label{eq:equiv_iv_opt_dtr}
  \Qfunc^\pi_{\vec{\lambda}, k} = \Qfunc^\pi_{\scrP, k}, \qquad \Vfunc^\pi_{\vec{\lambda}, k} = \Vfunc^\pi_{\scrP, k}, ~~\forall k\in[K].
  \end{equation}
  \item Reversely, if we fix any collection of prior distributions $\{\scrP_{\vec\bsh_k, a_k}\}$, then there exists a collection of weighting functions $\{\lambda_k(\vec\bsh_k, a_k)\}$ such that the above display holds true.
\end{enumerate}
 % and any collection of prior distributions $\{\scrP_{\vec\bsH_k, a_k}\}$.
% and construct $\{\underline Q^\pi_{\vec{\lambda}, k}, \overline Q^\pi_{\vec{\lambda}, k}$ as in Definition \ref{def:worst/best Q and value function} recursively for $k\in [K]$\footnote{For notational simplicity, we write $\underline{\Qfunc}_{K} = \underline{\Qfunc}_{\vec{\lambda}, K}^\pi$ and $\overline{\Qfunc}_{K} = \overline{\Qfunc}_{\vec{\lambda}, K}^\pi$, although they have no dependence on $\lambda$ and $\pi$. }.
% $\underline Q^\pi_{\vec{\lambda}, k}$ and $\overline Q^\pi_{\vec{\lambda}, k}$ are attained for $k\in [K]$. 
\end{theorem}

The above theorem effectively translates the problem of specifying a collection of prior distributions to specifying a collection of weighting functions, thus allowing one to bypass the integration over the prior distributions. This theorem, along with the dynamic programming algorithm presented in Theorem \ref{thm:iv_opt_dtr_dynamic_prog}, leads to the following alternative characterization of the IV-optimal DTR.

\begin{corollary}[Alternative characterization of the IV-optimal DTR]
\label{cor:struc_of_iv-opt_dtr}
Under the setting in Part 1 of Theorem \ref{thm:struc_of_iv-opt_dtr}, if we recursively define $\pi^\star$ as
\begin{equation}
  \label{eq:struc_of_iv-opt_dtr}
  \pi^\star_k(\vec\bsh_k) = \sgn\left\{\contr^{\pi^\star}_{\vec \lambda, k}(\vec\bsh_k) \right\} = \sgn\left\{Q_{\vec{\lambda}, k}^{\pi^\star}(\vec\bsh_k, +1) - Q_{\vec{\lambda}, k}^{\pi^\star}(\vec\bsh_k, -1) \right\}, ~~ k = K, K - 1, \hdots, 1,
\end{equation}  
where the two quantities
\begin{align}
  \label{eq:lb_wted_cate}
  Q_{\vec{\lambda}, k}^{\pi^\star}(\vec\bsh_k, +1)
  & = \lambda_k(\vec\bsh_k, +1) \cdot \underline{\Qfunc}_{\vec{\lambda} ,k}^{\pi^\star} (\vec\bsh_k, +1) + \big(1-\lambda_k(\vec\bsh_k, +1)\big) \cdot \overline{\Qfunc}_{\vec{\lambda}, k}^{\pi^\star} (\vec\bsh_k, +1),\\
  \label{eq:ub_wted_cate}
  Q_{\vec{\lambda}, k}^{\pi^\star}(\vec\bsh_k, -1)
  & = \lambda_k(\vec\bsh_k, -1) \cdot \underline{\Qfunc}_{\vec{\lambda}, k}^{\pi^\star} (\vec\bsh_k, -1) + \big(1-\lambda_k(\vec\bsh_k, -1)\big) \cdot \overline{\Qfunc}_{\vec{\lambda}, k}^{\pi^\star} (\vec\bsh_k, -1) 
\end{align}
depend on $\pi^\star$ only through $\pi^\star_{(k+1):K}$ and are therefore well-defined, then $\pi^\star$ satisfies \eqref{eq:iv_opt_dtr_k} for any stage $k$ and any configuration of the historical information $\vec\bsh_k$.
In particular, $\pi^\star$ is an IV-optimal DTR in the sense of Definition \ref{def:IV-Optimal DTR} when $\Pi$ consists of all Boolean functions.
\end{corollary}

% that for any collection of prior distributions $\big\{\scrP_{\vec\bsh_k, a_k}, 1 \leq k\leq K\big\}$, there exists a sequence of constants $\{\lambda_k(\vec\bsh_k, a_k),~k\in [K]\}\subseteq [0, 1]^K$ such that the weighted Q-functions and corresponding value functions at each stage $k \in [K]$ agree with the IV-constrained $Q$-functions and corresponding value functions in Definition \ref{def:DTR IV-constrained Q and value function}. Moreover, the reverse is also true so that specifying a sequence of priors $\big\{\scrP_{\vec\bsh_k, a_k}, k\in [K]\big\}$ is equivalent to specifying a sequence of constants $\{\lambda_k(\vec\bsh_k, a_k),~k\in [K]\}\subseteq [0, 1]^K$ in the sense that the collection of all IV-constrained $Q$-functions $\Qfunc^\pi_{\scrP, k}$'s (resp. $\Vfunc^\pi_{\scrP, k}$'s) in Definition \ref{def:DTR IV-constrained Q and value function} is the same as the collection of all weighted Q-functions $\Qfunc^\pi_{\vec{\lambda}, k}$'s (resp. $\Vfunc^\pi_{\vec{\lambda}, k}$'s) in Definition \ref{def:worst/best Q and value function}. 

% \sxc{This theorem is a bit too long, maybe split it into one theorem (the equivalence part) and one corollary (the formula, and this is a corollary of both this theorem and the theorem in the previous section).}


Compared to Theorem \ref{thm:iv_opt_dtr_dynamic_prog}, Corollary \ref{cor:struc_of_iv-opt_dtr} gives an alternative, analytic and constructive characterization of the IV-optimal DTR. 


\paragraph{An illustrative example when $K=2$.}
Figure \ref{fig: illustrate two stages} illustrates the decision process when $K = 2$. At the second stage, given $\vec{\bsh}_2^+ = ({\bsh}_1, a_1=+1, R_1(+1) = r_1^+, \bsX_2(+1) = \bsx_2^+)$ 
% (or $\vec{\bsh}'_2 = (\vec{\bsh}_1, a_1 = -1, R_1(-1) \mid \vec{\bsh}_1)$) 
and $\lambda_2(\vec\bsh_2^+, \pm 1)$, an IV-optimal action is made based on comparing two weighted $Q$-functions $Q_{\vec\lambda, 2}(\vec\bsh_2^+, +1) = 0.8$ and $Q_{\vec\lambda, 2}(\vec\bsh_2^+, -1) = 0.5$. Since $0.8>0.5$, we have $\pi^\star_2(\vec\bsh_2^+) = +1$. 
% From the figure, since 
The decision given $\vec\bsh_2^- = (\bsh_1, a_1 = -1, R_1(-1) = r_1^-, \bsX_2(-1) = \bsx_2^-)$ and $\lambda_2(\vec\bsh_2^-, \pm 1)$ is similar, and we have $\pi^\star_2(\vec\bsh_2^-) = -1$ in this case.

\begin{figure}[t!]
    \centering
    \begin{tikzpicture}[scale=0.6, every text node part/.style={align=center},
    node distance=2cm]
% nodes

% Stage 1
\draw[gray, ultra thick] (-2,0) -- (2,3);
\draw[red, ultra thick] (-2,0) -- (2,-3);
\filldraw[black] (-2,0) circle (2pt);
\node at (-2.5, 0) {${\bsh_1}$};
\node[align=left] at (-0.6,2.1) {\small $a_1 = +1$};
\node[align=left] at (-0.6,-2.2) {\small $a_1 = -1$};
\draw[|-|, ultra thick] (2,2) -- (2,4);
\draw[|-|, ultra thick] (2,-2) -- (2,-4);

\node at (4.2, 6) {\small${\Qfunc}_{\vec\lambda, 1}^{\pi^\star} (\bsh_1, +1) =\textcolor{black}{1.6} $};
\node at (4.2, 4) {\small $\overline{\Qfunc}^{\pi^\star}_{\vec{\lambda}, 1} (\bsh_1, +1) $};
\node at (4.2, 2) {\small $\underline{\Qfunc}^{\pi^\star}_{\vec{\lambda}, 1} (\bsh_1, +1)  $};

\node at (4.2, -2) {\small $\overline{\Qfunc}^{\pi^\star}_{\vec{\lambda}, 1} (\bsh_1, +1)  $};
\node at (4.2, -4) {\small $\underline{\Qfunc}^{\pi^\star}_{\vec{\lambda}, 1} (\bsh_1, +1)  $};
\node at (4.2, -6) {\small${\Qfunc}_{\vec\lambda, 1}^{\pi^\star} (\bsh_1, -1) =\textcolor{red}{1.9} $};

% Stage 2
\draw[-, gray, ultra thick, dashed] (2, 3) -- (8, 3);
\draw[-, gray, ultra thick, dashed] (2, -3) -- (8, -3);

\filldraw[black] (8, 3) circle (2pt);
\node at (7.5, 3.5) {$\vec{\bsh}_2^+$};
\draw[red, ultra thick] (8,3) -- (10.7,5);
\draw[gray, ultra thick] (8,3) -- (10.7,1);
\draw[|-|, ultra thick] (10.7,4.5) -- (10.7,5.5);
\draw[|-|, ultra thick] (10.7,0.5) -- (10.7,1.5);
\node[align=left] at (8.8,4.6) {\small $a_2 = +1$};
\node[align=left] at (8.8,1.4) {\small $a_2 = -1$};
\node at (12.8, 5.5) {\small$\overline{\Qfunc}_{2} (\vec\bsh_2^+, +1)$};
\node at (18, 5) {\small${\Qfunc}_{\vec\lambda, 2} (\vec\bsh_2^+, +1) =\textcolor{red}{0.8} $};
\node at (12.8, 4.5) {\small$\underline{\Qfunc}_{2} (\vec\bsh_2^+, +1)  $};
\node at (12.8, 1.5) {\small$\overline{\Qfunc}_{2} (\vec\bsh^+_2, -1)  $};
\node at (18, 1) {\textcolor{black}{\small${\Qfunc}_{\vec\lambda, 2} (\vec\bsh_2^+, -1) = 0.5  $}};
\node at (12.8, 0.5) {\small$\underline{\Qfunc}_{2}(\vec\bsh^+_2, -1)  $};

\filldraw[black] (8, -3) circle (2pt);
\node at (7.5, -3.5) {$\vec{\bsh}^-_2$};
\draw[red, ultra thick] (8,-3) -- (10.7,-5);
\draw[gray, ultra thick] (8,-3) -- (10.7,-1);
\draw[|-|, ultra thick] (10.7,-4.5) -- (10.7,-5.5);
\draw[|-|, ultra thick] (10.7,-0.5) -- (10.7,-1.5);
\node[align=left] at (8.8,-4.6) {\small $a_2 = -1$};
\node[align=left] at (8.8,-1.4) {\small $a_2 = +1$};
\node at (12.8, -4.5) {\small$\overline{ \Qfunc}_{2} (\vec\bsh^-_2, -1)  $};
\node at (18, -5) {\small${\Qfunc}_{\vec\lambda, 2} (\vec\bsh_2^-, -1) =\textcolor{red}{0.9} $};
\node at (12.8, -5.5) {\small$\underline{\Qfunc}_{2} (\vec\bsh^-_2, -1)  $};
\node at (12.8, -0.5) {\small$\overline{ \Qfunc}_{2} (\vec\bsh^-_2, +1)  $};
\node at (18, -1) {\small${\Qfunc}_{\vec\lambda, 2} (\vec\bsh_2^-, +1) =\textcolor{black}{0.7} $};
\node at (12.8, -1.5) {\small$\underline{\Qfunc}_{2} (\vec\bsh^-_2, +1)  $};

\end{tikzpicture}
\caption{
\small
An illustrative example of an IV-optimal DTR when $K=2$. 
According to the values of the weighted $Q$-functions at the second stage, we have $\pi^\star_2(\vec\bsh_2^+) = +1$ and $\pi^\star_2(\vec\bsh_2^-)= -1$.
Given $\pi^\star_2$, the weighted $Q$-functions at the first stage can be computed, and the IV-optimal action is $\pi^\star_1(\bsh_1) = -1$.
% as $Q_{\vec\lambda, 2}(\vec\bsh_2^+, +1) > Q_{\vec\lambda, 2}(\vec\bsh_2^+, -1)$.
% The stage-$2$ information $\vec{\bsh}_2 = (\vec{\bsh}_1, a_1 = + 1, R_1(+1) \mid \vec{\bsh}_1)$ and $\vec{\bsh}'_2 = (\vec{\bsh}_1, a_1 = -1, R_1(-1) \mid \vec{\bsh}_1)$. The superscript $\pi^\star$ of stage-$1$ Q-functions represent their dependence on the IV-optimal stage-$2$ decision rule. The stage-$1$ interval $\big[\underline{\Qfunc}^{\pi^\star}_{\vec{\lambda}, 2} (\vec\bsh_2, +1), \overline{\Qfunc}^{\pi^\star}_{\vec{\lambda}, 2} (\vec\bsh_2, +1)\big]$ is the partial identification interval of the cumulative rewards of interest when we take $a_1 = +1$ and set $a_2$ to the optimal decision rule according to $\vec{\bsh}_2 = (\vec{\bsh}_1, a_1 = + 1, R_1(+1) \mid \vec{\bsh}_1)$}
}
\label{fig: illustrate two stages}
\end{figure}






Given the knowledge of $\pi^\star_2$, we can compute the weighted value function $V^{\pi^\star}_{\vec\lambda, 2}(\cdot)$ of $\pi^\star$ at the second stage.
% Let $\pi^\star_2$ denote the IV-optimal decision at the second stage and $V_2^{\pi^\star}(\vec{\bsh}_2)$ the corresponding value. 
% Importantly, $V_2^{\pi^\star}(\vec{\bsh}_2)$ is a function of the first-stage covariate $\bsh_1$ and first-stage reward $R_1(a_1)$, because 
 % conditional on $\vec{\bsh}_1$, and depends on $\lambda_2(\vec\bsh_2, \pm 1)$ and $\pi^\star_2$.
This allows us to construct a ``pseudo-outcome'' at the first stage, denoted as $PO_1(r_1, \bsx_2|{\bsh}_1, a_1) = r_1 + V_2^{\pi^\star}({\bsh}_1, a_1, r_1, \bsx_2)$.
Importantly, $PO_1$ depends on $\pi^\star_2$, as it is the cumulative rewards if we observe $\bsh_1$ at the first stage, take an immediate action $a_1$, and then act according to the IV-optimal decision $\pi^\star_2$ at the second stage. 
% at the first stage if we were to act $a_2 = \pi^\star_2(\cdot)$



The partial identification interval for the expected value of $PO_1(R_1(a_1), \bsX_2(a_1)|\bsh_1, a_1)$, where the expectation is taken over the potential outcome distribution of $R_1(a_1)$ and $\bsX_2(a_1)$, is precisely the worst-case and best-case $Q$-functions $\underline{Q}^{\pi^\star}_{\vec\lambda, 1}(\bsh_1, a_1)$ and $\overline{Q}^{\pi^\star}_{\vec\lambda, 1}(\bsh_1, a_1)$. To this end, we can compute the weighted $Q$-function $Q^{\pi^\star}_{\vec\lambda,1}(\bsh_1, a_1)$ if $\lambda_1(\bsh_1, a_1)$ is specified, from which we can decide $\pi^\star_1$. Reading the numbers off Figure \ref{fig: illustrate two stages}, we conclude that $\pi^\star_1(\bsh_1) = -1$.

% At the first stage, the best-case and worst-case Q-functions $\overline{\Qfunc}_{\vec{\lambda}, 1} (\bsh_1, +1)$ and $\underline{\Qfunc}_{\vec{\lambda}, 1} (\bsh_1, +1)$ are estimating the upper and lower bounds of the expected \emph{cumulative} rewards if we were to let $a_1 = +1$ and $a_2 = \pi_2^\star(\vec{\bsh}_2)$. 
% In other words, they are bounds on the expectation (conditional on $\vec{\bsh}_1$) of the pseudo-outcome $PO_1(\vec{\bsh}_1, +1) := R_1(+1) + V_2^{\pi^\star}(\vec{\bsh}_2)= R_1(+1) + V_2^{\pi^\star}(\vec{\bsh}_1, a_1 = +1, R_1(+1))$. Similarly, $\overline{\Qfunc}_{\vec{\lambda}, 1} (\bsh_1, -1)$ and $\underline{\Qfunc}_{\vec{\lambda}, 1} (\bsh_1, -1)$ are partial identification intervals of the pseudo-outcome $PO_1(\vec{\bsh}_1, -1) := R_1(-1) + V_2^{\pi^\star}(\vec{\bsh}_1, a_1 = -1, R_1(-1))$. The first-stage decision is again made based on an interplay between four action value functions $\overline{\Qfunc}_{\vec{\lambda}, 1} (\bsh_1, \pm 1)$ and $\underline{\Qfunc}_{\vec{\lambda}, 1} (\bsh_1, \pm 1)$ for specified constants $\lambda_1(\vec{\bsh}_1, \pm 1)$.






%%%%%% BELOW IS AN IMPLEMENTATION USING MINIPAGE IN THE SUBFIG PACKAGE %%%%%%%
% \begin{figure}[t!]
%     \centering
%     \begin{minipage}{0.45\textwidth}
%     \subfloat[][\small Worst-Case: $\lambda_k(\vec\bsh_k, +1) = \lambda_k(\vec\bsh_k, -1) = 1$.]{
%     \begin{tikzpicture}[scale=0.6, node distance=2cm]
% % nodes
% \draw[gray, ultra thick, red] (0,0) -- (3,2);
% \draw[gray, ultra thick] (0,0) -- (3,-2);
% \filldraw[black] (0,0) circle (2pt);
% \node at (-0.5, 0) {$\vec{\bsh_k}$};
% \node[align=left] at (1.2,1.8) {\small $a_k = +1$};
% \node[align=left] at (1.2,-1.8) {\small $a_k = -1$};
% \draw[|-|, ultra thick] (3,1) -- (3,3);
% \draw[|-|, ultra thick] (3,-1) -- (3,-3);
% \node at (6.3, 1) {$\underline{\Qfunc}_{\vec{\lambda} ,k}^{\pi} (\vec\bsh_k, +1) = 1.0$};
% \node at (6.3, 3) {$\overline{\Qfunc}_{\vec{\lambda} ,k}^{\pi} (\vec\bsh_k, +1) = 1.5$};
% \node at (6.3, -1) {$\overline{\Qfunc}_{\vec{\lambda} ,k}^{\pi} (\vec\bsh_k, -1) = 5.0$};
% \node at (6.3, -3) {$\underline{\Qfunc}_{\vec{\lambda} ,k}^{\pi} (\vec\bsh_k, -1) = 0.8$};
% \filldraw[red] (3, 1) circle (3pt);
% \filldraw[red] (3, -3) circle (3pt);
% \end{tikzpicture}}
%     \end{minipage}\hspace{1.5cm}


%     \begin{minipage}{0.45\textwidth}
%      \subfloat[][\small Best-Case: $\lambda_k(\vec\bsh_k, +1) = \lambda_k(\vec\bsh_k, -1) = 0$.]{
%     \begin{tikzpicture}[scale=0.6, node distance=2cm]
% % nodes
% \draw[gray, ultra thick] (0,0) -- (3,2);
% \draw[gray, ultra thick, red] (0,0) -- (3,-2);
% \filldraw[black] (0,0) circle (2pt);
% \node at (-0.5, 0) {$\vec{\bsh_k}$};
% \node[align=left] at (1.2,1.8) {\small $a_k = +1$};
% \node[align=left] at (1.2,-1.8) {\small $a_k = -1$};
% \draw[|-|, ultra thick] (3,1) -- (3,3);
% \draw[|-|, ultra thick] (3,-1) -- (3,-3);
% \node at (6.3, 1) {$\underline{\Qfunc}_{\vec{\lambda} ,k}^{\pi} (\vec\bsh_k, +1) = 1.0$};
% \node at (6.3, 3) {$\overline{\Qfunc}_{\vec{\lambda} ,k}^{\pi} (\vec\bsh_k, +1) = 1.5$};
% \node at (6.3, -1) {$\overline{\Qfunc}_{\vec{\lambda} ,k}^{\pi} (\vec\bsh_k, -1) = 5.0$};
% \node at (6.3, -3) {$\underline{\Qfunc}_{\vec{\lambda} ,k}^{\pi} (\vec\bsh_k, -1) = 0.8$};
% \filldraw[red] (3, 3) circle (3pt);
% \filldraw[red] (3, -1) circle (3pt);
% \end{tikzpicture}}
%     \end{minipage}\\ \vspace{2 cm}


%     \begin{minipage}{0.45\textwidth}
%     \subfloat[][\small Min-Max: $\lambda_k(\vec\bsh_k, +1) = \lambda_k(\vec\bsh_k, -1) = 1/2$. ]{
%     \begin{tikzpicture}[scale=0.6, node distance=2cm]
% % nodes
% \draw[gray, ultra thick] (0,0) -- (3,2);
% \draw[gray, ultra thick, red] (0,0) -- (3,-2);
% \filldraw[black] (0,0) circle (2pt);
% \filldraw[red] (3, 2) circle (3pt);
% \filldraw[red] (3, -2) circle (3pt);
% \node at (-0.5, 0) {$\vec{\bsh_k}$};
% \node[align=left] at (1.2,1.8) {\small $a_k = +1$};
% \node[align=left] at (1.2,-1.8) {\small $a_k = -1$};
% \draw[|-|, ultra thick] (3,1) -- (3,3);
% \draw[|-|, ultra thick] (3,-1) -- (3,-3);
% \node at (6.3, 1) {$\underline{\Qfunc}_{\vec{\lambda} ,k}^{\pi} (\vec\bsh_k, +1) = 1.0$};
% \node at (6.3, 3) {$\overline{\Qfunc}_{\vec{\lambda} ,k}^{\pi} (\vec\bsh_k, +1) = 1.5$};
% \node at (6.3, -1) {$\overline{\Qfunc}_{\vec{\lambda} ,k}^{\pi} (\vec\bsh_k, -1) = 5.0$};
% \node at (6.3, -3) {$\underline{\Qfunc}_{\vec{\lambda} ,k}^{\pi} (\vec\bsh_k, -1) = 0.8$};
% \end{tikzpicture}}
%     \end{minipage}\hspace{1cm}
%     \begin{minipage}{0.45\textwidth}
%      \subfloat[][User-Specific: $\lambda_k(\vec\bsh_k, +1) = 1/4, ~\lambda_k(\vec\bsh_k, -1) = 5/6$]{
%     \begin{tikzpicture}[scale=0.6, node distance=2cm]
% % nodes
% \draw[gray, ultra thick] (0,0) -- (3,2);
% \draw[gray, ultra thick, red] (0,0) -- (3,-2);
% \filldraw[black] (0,0) circle (2pt);
% \filldraw[red] (3, 1.5) circle (3pt);
% \filldraw[red] (3, -1.33) circle (3pt);
% \node at (-0.5, 0) {$\vec{\bsh_k}$};
% \node[align=left] at (1.2,1.8) {\small $a_k = +1$};
% \node[align=left] at (1.2,-1.8) {\small $a_k = -1$};
% \draw[|-|, ultra thick] (3,1) -- (3,3);
% \draw[|-|, ultra thick] (3,-1) -- (3,-3);
% \node at (6.3, 1) {$\underline{\Qfunc}_{\vec{\lambda} ,k}^{\pi} (\vec\bsh_k, +1) = 1.0$};
% \node at (6.3, 3) {$\overline{\Qfunc}_{\vec{\lambda} ,k}^{\pi} (\vec\bsh_k, +1) = 1.5$};
% \node at (6.3, -1) {$\overline{\Qfunc}_{\vec{\lambda} ,k}^{\pi} (\vec\bsh_k, -1) = 5.0$};
% \node at (6.3, -3) {$\underline{\Qfunc}_{\vec{\lambda} ,k}^{\pi} (\vec\bsh_k, -1) = 0.8$};
% \end{tikzpicture}}
%     \end{minipage}
%     \caption{\small Stage-$k$ decision making corresponding to different choices of $\lambda_k(\vec\bsh_k, \pm 1)$. Corresponding weighted Q-functions are represented by red dots in each arm. Top left panel corresponds to a worst-case perspective and letting $a_k = \text{sgn}\big\{\underline{\Qfunc}_{\vec{\lambda} ,k}^{\pi} (\vec\bsh_k, +1) - \underline{\Qfunc}_{\vec{\lambda} ,k}^{\pi} (\vec\bsh_k, -1)\big\} = \text{sgn}\{1 - 0.8\} = +1$. Top right panel corresponds to a best-case perspective and letting $a_k = \text{sgn}\big\{\overline{\Qfunc}_{\vec{\lambda} ,k}^{\pi} (\vec\bsh_k, +1) - \overline{\Qfunc}_{\vec{\lambda} ,k}^{\pi} (\vec\bsh_k, -1)\big\} = \text{sgn}\{1.5 - 5.0\} = -1$. 
%     Bottom left panel corresponds to a min-max perspective and letting $a_k = \text{sgn}\big\{\overline{\Qfunc}_{\vec{\lambda} ,k}^{\pi} (\vec\bsh_k, +1) + \underline{\Qfunc}_{\vec{\lambda} ,k}^{\pi} (\vec\bsh_k, +1) - \big(\overline{\Qfunc}_{\vec{\lambda} ,k}^{\pi} (\vec\bsh_k, -1) + \underline{\Qfunc}_{\vec{\lambda} ,k}^{\pi} (\vec\bsh_k, -1)\big)\big\} = \text{sgn}\{1.5 + 1.0 - (5.0+0.8)\} = -1$. Bottom right panel corresponds to a user-specified choice of $\lambda_k(\vec\bsh_k, +1) = 1/4$ and $\lambda_k(\vec\bsh_k, -1) = 5/6$, and $a_k = \text{sgn}\big\{\big(1/4 \cdot\overline{\Qfunc}_{\vec{\lambda} ,k}^{\pi} (\vec\bsh_k, +1) +3/4\cdot \underline{\Qfunc}_{\vec{\lambda} ,k}^{\pi} (\vec\bsh_k, +1)\big) - \big(5/6\cdot\overline{\Qfunc}_{\vec{\lambda} ,k}^{\pi} (\vec\bsh_k, -1) + 1/6\cdot \underline{\Qfunc}_{\vec{\lambda} ,k}^{\pi} (\vec\bsh_k, -1)\big)\big\} = \text{sgn}\{(1/4 \cdot 1.5 + 3/4\cdot 1.0) - (5/6\cdot 5.0 + 1/6\cdot 0.8)\} = -1$.}
%     \label{fig: illustrate stage k}
% \end{figure}


%%%%%% BELOW IS AN IMPLEMENTATION USING SUBFIGURE IN THE SUBCAPTION PACKAGE %%%%%%%
\begin{figure}[t!]
\centering
% FIGURE AT LOCATION [0, 0] 
\begin{subfigure}[b]{0.30\textwidth}
  \centering
  \begin{tikzpicture}[scale=0.6, node distance=2cm]
  \draw[gray, ultra thick, red] (0,0) -- (2,3);
  \draw[gray, ultra thick] (0,0) -- (2,-3);
  \filldraw[black] (0,0) circle (2pt);
  \node at (-0.5, 0) {\small $\vec{\bsh_k}$};
  \node[align=left] at (0.5,1.8) {\small $+1$};
  \node[align=left] at (0.5,-1.8) {\small $-1$};
  \draw[|-|, ultra thick] (2,2) -- (2,4);
  \draw[|-|, ultra thick] (2,-2) -- (2,-4);
  \node at (2.5, 5.5) {\small ${\Qfunc}^{\pi^\star}_{\vec\lambda, k} (\vec\bsh_k, +1) =\textcolor{red}{1.0} $};
  \node at (5.3, 2) {\small $\underline{\Qfunc}_{\vec{\lambda} ,k}^{ \pi^\star} (\vec\bsh_k, +1) = 1.0$};
  \node at (5.3, 4) {\small $\overline{\Qfunc}_{\vec{\lambda} ,k}^{  \pi^\star} (\vec\bsh_k, +1) = 1.5$};
  \node at (5.3, -2) {\small $\overline{\Qfunc}_{\vec{\lambda} ,k}^{ \pi^\star} (\vec\bsh_k, -1) = 5.0$};
  \node at (5.3, -4) {\small $\underline{\Qfunc}_{\vec{\lambda} ,k}^{\pi^\star} (\vec\bsh_k, -1) = 0.8$};
  \node at (2.5,  -5.5) {\small ${\Qfunc}^{\pi^\star}_{\vec\lambda, k} (\vec\bsh_k, -1) =\textcolor{black}{0.8} $};
  \filldraw[red] (2, 2) circle (3pt);
  \filldraw[red] (2, -4) circle (3pt);
  \end{tikzpicture}
  \caption[]
  {{\footnotesize Worst-Case: $\lambda_k(\vec\bsh_k, \pm 1) = 1$.}}
  \label{fig: illustrate stage k worst case}
\end{subfigure}
\hfill
% FIGURE AT LOCATION [0, 1] 
\begin{subfigure}[b]{0.3\textwidth}  
  \centering 
  \begin{tikzpicture}[scale=0.6, node distance=2cm]
  \draw[gray, ultra thick] (0,0) -- (2,3);
  \draw[gray, ultra thick, red] (0,0) -- (2,-3);
  \filldraw[black] (0,0) circle (2pt);
  \node at (-0.5, 0) {\small $\vec{\bsh_k}$};
  \node[align=left] at (0.5,1.8) {\small $+1$};
  \node[align=left] at (0.5,-1.8) {\small $-1$};
  \draw[|-|, ultra thick] (2,2) -- (2,4);
  \draw[|-|, ultra thick] (2,-2) -- (2,-4);
  \node at (2.5,  5.5) {\small ${\Qfunc}^{\pi^\star}_{\vec\lambda, k} (\vec\bsh_k, +1) =\textcolor{black}{1.5} $};
  \node at (5.3, 2) {\small $\underline{\Qfunc}_{\vec{\lambda} ,k}^{ \pi^\star} (\vec\bsh_k, +1) = 1.0$};
  \node at (5.3, 4) {\small $\overline{\Qfunc}_{\vec{\lambda} ,k}^{  \pi^\star} (\vec\bsh_k, +1) = 1.5$};
  \node at (5.3, -2) {\small $\overline{\Qfunc}_{\vec{\lambda} ,k}^{ \pi^\star} (\vec\bsh_k, -1) = 5.0$};
  \node at (5.3, -4) {\small $\underline{\Qfunc}_{\vec{\lambda} ,k}^{\pi^\star} (\vec\bsh_k, -1) = 0.8$};
  \node at (2.5, -5.5) {\small ${\Qfunc}^{\pi^\star}_{\vec\lambda, k} (\vec\bsh_k, -1) =\textcolor{red}{5.0} $};
  \filldraw[red] (2, 2) circle (3pt);
  \filldraw[red] (2, -2) circle (3pt);
  \end{tikzpicture}
  \caption[]%
  {{\footnotesize Best-Case: $\lambda_k(\vec\bsh_k, \pm 1) = 0$.}}
  \label{fig: illustrate stage k best case}
 \end{subfigure}
 \hfill
% FIGURE LOCATED AT [1, 0]
\begin{subfigure}[b]{0.3\textwidth}   
  \centering 
  \begin{tikzpicture}[scale=0.6, node distance=2cm]
  \draw[gray, ultra thick] (0,0) -- (2,3);
  \draw[gray, ultra thick, red] (0,0) -- (2,-3);
  \filldraw[black] (0,0) circle (2pt);
  \node at (-0.5, 0) {\small $\vec{\bsh_k}$};
  \node[align=left] at (0.5,1.8) {\small $+1$};
  \node[align=left] at (0.5,-1.8) {\small $-1$};
  \draw[|-|, ultra thick] (2,2) -- (2,4);
  \draw[|-|, ultra thick] (2,-2) -- (2,-4);
  \filldraw[red] (2, 3) circle (3pt);
  \filldraw[red] (2, -3) circle (3pt);
  \node at (2.5,  5.5) {\small ${\Qfunc}^{\pi^\star}_{\vec\lambda, k} (\vec\bsh_k, +1) =\textcolor{black}{1.25} $};
  \node at (5.3, 2) {\small $\underline{\Qfunc}_{\vec{\lambda} ,k}^{\pi^\star} (\vec\bsh_k, +1) = 1.0$};
  \node at (5.3, 4) {\small $\overline{\Qfunc}_{\vec{\lambda} ,k}^{ \pi^\star} (\vec\bsh_k, +1) = 1.5$};
  \node at (5.3, -2) {\small $\overline{\Qfunc}_{\vec{\lambda} ,k}^{\pi^\star} (\vec\bsh_k, -1) = 5.0$};
  \node at (5.3, -4) {\small $\underline{\Qfunc}_{\vec{\lambda},k}^{\pi^\star} (\vec\bsh_k, -1) = 0.8$};
  \node at (2.5,  -5.5) {\small ${\Qfunc}^{\pi^\star}_{\vec\lambda, k} (\vec\bsh_k, -1) =\textcolor{red}{2.90} $};
  \end{tikzpicture}
  \caption[]%
  {{\footnotesize Min-Max: $\lambda_k(\vec\bsh_k, \pm 1) =\frac{1}{2}$.}}
  \label{fig: illustrate stage k min max}
\end{subfigure}
% CAPTION AND LABELS FOR THE WHOLE FIGURE
\caption[]
{\small IV-optimal DTR at stage $k$ with different choices of weighting functions.
% $\lambda_k(\vec\bsh_k, \pm 1)$. 
The weighted $Q$-functions are represented by red dots in each arm, and the corresponding IV-optimal action is colored in red. Figure \ref{fig: illustrate stage k worst case} corresponds to the worst-case perspective, Figure \ref{fig: illustrate stage k best case} the best-case perspective, and Figure \ref{fig: illustrate stage k min max} the min-max perspective. In each case, the IV-optimal action is $\sgn\{Q_{\vec{\lambda}, k}^{\pi^\star}(\vec\bsh_k, +1) - Q_{\vec{\lambda}, k}^{\pi^\star}(\vec\bsh_k, -1) \}$.} 
\label{fig: illustrate stage k}
\end{figure}

\paragraph{Choice of the weighting functions.}
% \begin{remark}[Choosing $\lambda_k(\vec{\bsh}_k, a_k)$]\label{remark: DTR choose lambda}\rm
%We conclude this subsection with a remark on the choice of weighting functions.
% Corollary \ref{cor:struc_of_iv-opt_dtr} makes choosing the stage-$k$ constant $\lambda_k(\vec\bsh_{k}, a_k)$ very transparent. 
The specification of weighting functions reveals one's level of optimism.
Suppose that the future weighting functions $\{\lambda_t: t\geq k+1\}$ has been specified. At stage $k$, if one adopts a worst-case perspective and would like to maximize the worst-case gain at this stage (fixing the weighting function specifications at all future stages),
% (fixing future constants $\{\lambda_t(\vec\bsh_{t}, a_t),~k+1 \leq t \leq K\}$), 
then it suffices to compare the two worse-case Q-functions at stage $k$, namely $\underline{\Qfunc}_{\vec{\lambda} ,k}^{\pi^\star} (\vec\bsh_k, +1)$ and $\underline{\Qfunc}_{\vec{\lambda} ,k}^{\pi^\star} (\vec\bsh_k, -1)$.
And the pessimistic action is taken to be sign of the difference of the two worst-case $Q$-functions,
% $a_k = \text{sgn}\big\{\underline{\Qfunc}_{\vec{\lambda} ,k}^{\pi} (\vec\bsh_k, +1) - \underline{\Qfunc}_{\vec{\lambda} ,k}^{\pi} (\vec\bsh_k, -1)\big\}$, 
which corresponds to taking $\lambda_k(\vec\bsh_k, \pm 1) = 1$ (see Figure \ref{fig: illustrate stage k worst case}). Alternatively, if one adopts a best-case perspective at stage $k$ and would like to maximize the best-case gain at this stage, then one shall compare the two best-case $Q$-functions, namely $\overline{\Qfunc}_{\vec{\lambda} ,k}^{\pi^\star} (\vec\bsh_k, +1)$ and $\overline{\Qfunc}_{\vec{\lambda} ,k}^{\pi^\star} (\vec\bsh_k, -1)$. The optimistic action is then taken to be the difference between the two best-case $Q$-functions, which corresponds to taking $\lambda_k(\vec\bsh_k, \pm 1) = 0$ (see Figure \ref{fig: illustrate stage k best case}). Recall that in the single-stage setting, the min-max risk criterion \ref{eq:worst_case_risk_single_stage} corresponds to maximizing the weighted value \eqref{eqn: middle ground of value interval} with weights set to be $1/2$. This criterion can be seamlessly generalized to the current multiple-stage setting by setting $\lambda_k(\vec\bsh_k, \pm 1)  = 1/2$ (see Figure \ref{fig: illustrate stage k min max}). Other choices of weighting functions can be made to incorporate domain knowledge and user preference, as suggested by \cite{cui2021machine}.

% Alternatively, one may first form the partial identification interval for the contrast function at stage $k$, i.e., $\big[\underline{\Qfunc}_{\vec{\lambda} ,k}^{\pi} (\vec\bsh_k, +1) - \overline{\Qfunc}_{\vec{\lambda} ,k}^{\pi} (\vec\bsh_k, -1), \overline{\Qfunc}_{\vec{\lambda} ,k}^{\pi} (\vec\bsh_k, +1) - \underline{\Qfunc}_{\vec{\lambda} ,k}^{\pi} (\vec\bsh_k, -1)\big]$, and then minimize the maximum stage-$k$ risk by taking $a_k = \text{sgn}\big\{\overline{\Qfunc}_{\vec{\lambda} ,k}^{\pi} (\vec\bsh_k, +1) + \underline{\Qfunc}_{\vec{\lambda} ,k}^{\pi} (\vec\bsh_k, +1) - \big(\overline{\Qfunc}_{\vec{\lambda} ,k}^{\pi} (\vec\bsh_k, -1) + \underline{\Qfunc}_{\vec{\lambda} ,k}^{\pi} (\vec\bsh_k, -1)\big)\big\}$, which corresponds to taking $\lambda_k(\vec\bsh_k, +1) = \lambda_k(\vec\bsh_k, -1) = 1/2$ in \eqref{eq:struc_of_iv-opt_dtr}. These strategies have their counterparts in a single-stage ITR setting discussed in XX and reviewed in Section \ref{subsec: IV optimality review}. Figure \ref{fig: illustrate stage k} illustrates each strategy with a concrete example.
% \end{remark}

\subsection{Estimating an IV-Optimal DTR}
\label{subsec: estimate IV-optimal DTR}
% \sxc{Our algorithm bears similarities with the literature on ``policy distillation'', where the goal is to derive a simple policy from a complicated one while preserving the performance, maybe we can give our algorithm a name like ``distilled $Q$-learning. In terms of presentation we can divide into two parts: (1) first introduce a $Q$-learning algorithm (essentially we are estimating all the contrasts recursively), and then (2) introduce how to distill the policy learned by $Q$-learning via weighted classification (using the estimated contrasts).}

%The foregoing discussion has focused on how to obtain an IV-optimal DTR given the knowledge of certain population quantities. In this subsection, we present a strategy to estimate an IV-optimal DTR given i.i.d.~samples from the law of the random trajectory $(\bsX_k^\obs, A_k^\obs, R_k^\obs)_{k = 1}^K$ and the time-varying instrument variable $\{Z_k\}_{k=1}^K$.

We discuss how to estimate an IV-optimal DTR given i.i.d.~samples from the law of the random trajectory $(\bsX_k^\obs, A_k^\obs, R_k^\obs)_{k = 1}^K$ and a time-varying instrument variable $\{Z_k\}_{k=1}^K$. The IV-constrained sets $\{\calP_{\vec\bsh_k, a_k}\}$ are specified via partial identification intervals for the $Q$-functions. Specifically, let 
% \sxc{move it to earlier sections??}
\begin{align}
  \calP_{\vec\bsh_k, a_k}
  & = 
  \bigg\{
    p_{a_k}(\cdot, \cdot|\vec\bsh_k)
    % ~\bigg|~
    :
    \forall %\textnormal{ sufficiently regular }
    f \in \calF_k,~
    \exists~
    \underline{Q}(\vec\bsh_k, a_k; f),
    \overline{Q}(\vec\bsh_k, a_k; f) \nonumber \\
  & \qquad
    \textnormal{ s.t. }
    \underline{Q}(\vec\bsh_k, a_k; f) 
    \leq 
    \int f(r_k , \bsx_{k+1}) p_{a_k}(d r_k, d\bsx_{k+1}|\vec\bsh_k)
    \leq 
    \overline{Q}(\vec\bsh_k, a_k; f) \nonumber \\
\label{eq:IV_contrained_set_general}
  & \qquad
    \textnormal{ and }
    R_k\in[\underline{C}_k, \overline{C}_k] 
    \textnormal{ almost surely for }
    (R_k, \bsX_{k+1}) \sim p_{a_k}(\cdot, \cdot|\vec\bsh_k)
  \bigg\}.
\end{align}

The boundedness of $R_k$ ensures that partial identification intervals (e.g, Manski-Pepper bounds) have finite width. This is a plausible assumption in many applications \citep{swanson2018partial}.


%While we will provide the detailed form of $\calF_k$ as well as $\underline{Q}(\vec\bsh_k, a_k; f), \overline{Q}(\vec\bsh_k, a_k; f)$ in the final algorithm descriptions, we first take some time to explain the intuitions behind the above specification. 

At the final stage $K$, we take $\calF_K = \{\textnormal{Id}\}$, a singleton containing the identity function that sends $r_K$ to itself (note that $\bsX_{x+1}$ is a null quantity and thus disregarded). 
Then the lower and upper bounds, namely $\underline{Q}(\vec\bsh_k, a_K; \textnormal{Id}) = \underline{Q}_K(\vec\bsh_k, a_K)$ and $\overline{Q}(\vec\bsh_k, a_K; \textnormal{Id}) = \underline{Q}_K(\vec\bsh_k, a_K)$, are precisely the endpoints of the partial identification intervals (constructed using the IV $Z_K$) of the expected final-stage reward $R_K$, where the expectation is taken over the potential outcome distribution $R_K\sim p^\star_{a_K}(\cdot|\vec\bsh_k)$. 
By construction, we have $p^\star_{a_K}(\cdot|\vec\bsh_k) \in \calP_{\vec\bsh_k, a_K}$.

For $k\leq K-1$, we will take $\calF_k$ to be a class of properly defined functions (the specific forms will be specified later) of the current reward $r_k$ and the next-stage covariate $\bsx_{k+1}$. 
The lower and upper bounds $\underline{Q}(\vec\bsh_k, a_k; f), \overline{Q}(\vec\bsh_k, a_k; f)$ now constitute the partial identification intervals (constructed using the IV $Z_k$) of the expected value of $f(R_k, \bsX_{k+1})$, where the expectation is taken over the potential outcome distribution $(R_k, \bsX_{k+1})\sim p^\star_{a_k}(\cdot, \cdot|\bsh_k)$. By construction, we have $p^\star_{a_k}(\cdot, \cdot|\vec\bsh_k) \in \calP_{\vec\bsh_k, a_k}$.


% speci...fication of $\cal_F$ as well as the lower and the upper bounds is more complicated.
% This means that $\calP_{\vec\bsh_k, a_K}$ is the set of distributions so that the expected final stage reward 
% The exact specifications of the function $f$ as well as the lower and upper bound $\underline{Q}(\vec\bsh_k, a_k; f), \overline{Q}(\vec\bsh_k, a_k; f)$ will be 

Let $\{(\bsx_{k, i}, a_{k, i}, r_{k, i})_{k=1}^K \}_{i=1}^n$ denote the observed data.
Let $\bsh_{1, i}= \bsx_{1, i}$ be the baseline covariates for the $i$-th sample. 
For $2 \leq k \leq K$, let $\vec\bsh_{k, i}= (\vec a_{k-1, i}, \vec r_{k-1, i}, \vec\bsx_{k, i})$ be the historical information up to stage $k$ for the $i$-th sample. In addition, let $\{z_{k, i}\}_{i=1}^n$ denote the stage-$k$ IV data. 
% We assume that the weighting functions $\{\lambda(\vec\bsh_k, a_k)\}$ and hence the prior distributions $\{\scrP_{\vec\bsh_k, a_k}\}$ are specified.



%In addition, let $\{z_{k, i}\}_{i=1}^n \overset{i.i.d.}{\sim} \textnormal{Law}(Z_k)$ be the instrument variables at stage $k$.
%We assume that the weighting functions $\{\lambda(\vec\bsh_k, a_k)\}$, and hence the prior distributions $\{\scrP_{\vec\bsh_k, a_k}\}$, are specified.


\paragraph{Estimating the contrasts by $Q$-learning.}
Corollary \ref{cor:struc_of_iv-opt_dtr} shows that to estimate the IV-optimal DTR $\pi^\star$, it suffices to estimate the contrast functions $\{\contr^{\pi^\star}_{\vec\lambda, k}(\vec\bsh_k)\}$ defined in \eqref{eq:struc_of_iv-opt_dtr}, which in turn calls for estimating the weighted $Q$-functions $\{Q^{\pi^\star}_{\vec\lambda, k}(\vec\bsh_k, \pm 1)\}$.
We use a $Q$-learning approach to estimate the weighted $Q$-functions (\sxc{CITE}). 

For ease of exposition, we specify \eqref{eq:IV_contrained_set_general} via Manski-Pepper bounds \citep{manski1998monotone}. Generalization to other types of partial identification intervals is immediate. For Manski-Pepper bounds to hold, 
% we need the reward at each stage to be bounded, 
% We consider a concrete example of partial identification bounds and illustrate how to estimate $\widehat{Q}_{\vec{\lambda}, k, i}^{\widehat{\pi}^\star}(\vec\bsh_{k, i}, \pm 1)$.
% We consider a binary IV, a binary treatment, and a continuous but bounded reward at each stage. 
% Boundedness of the outcome 
% which is often a plausible assumption in many practical situations (\citealp{swanson2018partial}). 
we make the 
% Partial identification of the ATE (and similarly CATE) for a continuous but bounded outcome typically relies on the so-called 
\emph{mean exchangeability} assumption (\citealp{manski1990nonparametric, hernan2006instruments, swanson2018partial}) or a relaxed \emph{monotone instrumental variable} (MIV) assumption (\citealp{manski1998monotone}). The mean exchangeability assumption is automatically satisfied in a sequential randomized controlled trial with noncompliance.

At Stage $K$, define
% For instance, under the MIV assumption (\citealt{manski1998monotone}), we define: 
\begin{align*}
% \begin{split}
    & \psi_{K}(\vec{\bsh}_K, a_k, z_k; C)  = C \cdot \bbP(A_K^\obs = -a_k \mid Z_K = z_k, \vec{\bsH}_K^\obs = \vec\bsh_k) \nonumber \\
    \label{eq:mp_bound_psi}
    & ~~ + \mathbb{E}[R_K^\obs \mid \vec{\bsH}_K^\obs = \vec\bsh_k, Z_K = z_k, A_K^\obs = a_k]
    \cdot \bbP(A_K^\obs = a_k \mid \vec{\bsH}_K^\obs = \vec\bsh_k, Z_K = z).\numberthis
    % & \qquad + C \cdot \bbP(A_K^\obs = -a_k \mid Z_K = z_k, \vec{\bsH}_K^\obs = \vec\bsh_k)
% \end{split}
\end{align*}
% at stage $K$. 
Manski-Pepper bounds state that if $R_K \in [\underline{C}_K, \overline{C}_K]$ almost surely (with respect to $p^\star_{a_K}(\cdot|\vec\bsh_k)$), then its conditional mean potential outcome $\bbE_{R_K\sim p^\star_{a_K}(\cdot|\vec\bsh_k)}[R_K]$ is lower and upper bounded by
\begin{align*}
    & \bbP(Z_K = -1 |\vec{\bsH}_K^\obs= \vec\bsh_k) \cdot \psi_{K}(\vec{\bsh}_K, a_K, -1; \underline{C}_K) \\
    \label{eq:mp_lower_bound}
    & \qquad + \bbP(Z_K = +1 |\vec{\bsH}_K^\obs = \vec\bsh_k)\cdot 
    \big[\psi_{K}(\vec{\bsh}_K, a_K, -1; \underline{C}_K) \lor 
    \psi_{K}(\vec{\bsh}_K, a_K, +1; \underline{C}_K) \big]\numberthis\\
    \text{and}& \\
    & \bbP(Z_K = -1 |\vec{\bsH}_K^\obs = \vec\bsh_k) 
    \cdot 
    \big [\psi_{K}(\vec{\bsh}_K, a_K, -1; \overline{C}_K )
    \land 
    \psi_{K}(\vec{\bsh}_K, a_K, +1; \overline{C}_K )\big]\\
    % & \bbP(Z_K = -1 |\vec{\bsH}_K^\obs= \vec\bsh_k) \cdot \psi_{K}(\vec{\bsh}_K, a_K, -1; \underline{C}_K) \\
    \label{eq:mp_upper_bound}
    & \qquad + \bbP(Z_K = +1|\vec{\bsH}_K^\obs = \vec\bsh_k)\cdot \psi_{K}(R_K, a_K, +1 ; \vec{\bsh}_K; \overline{C}_K ),\numberthis
\end{align*}
where $\land$ and $\lor$ are shorthands for $\min$ and $\max$, and both bounds are tight. Therefore, as long as we take $\calF_K \supseteq \{\text{Id}\}$ when defining $\calP_{\vec\bsh_k, a_K}$ in \eqref{eq:IV_contrained_set_general}, 
% Theorem \ref{thm:struc_of_iv-opt_dtr} would hold. This means that 
the worst-case and best-case $Q$ functions at stage $K$ defined in \eqref{eq:worst Q stage K}--\eqref{eq:best Q stage K} can be set to \eqref{eq:mp_lower_bound} and \eqref{eq:mp_upper_bound}, respectively. Along with $\lambda_K(\vec\bsh_k, a_K)$ specifications, the construction of the stage-$K$ weighted $Q$-function $Q_{\vec\lambda, K}(\vec\bsh_k, a_K)$ is concluded.

Since both \eqref{eq:mp_lower_bound} and \eqref{eq:mp_upper_bound} are functionals of the observed data distribution, $Q_{\vec\lambda, K}(\vec\bsh_k, a_K)$ can be estimated from the data by fitting parametric models (e.g., linear models) or flexible machine learning models (e.g., regression trees and random forests), and then invoke the plug-in principle.

Given an estimate $\hat Q_{\vec\lambda, K}^\star$ of $Q_{\vec\lambda, K}$, 
we can estimate the contrast function $\contr_{\vec\lambda, K}(\vec\bsh_k)$ by $\hat \contr^\star_{\vec\lambda, K}(\vec\bsh_k) = \hat Q_{\vec\lambda, K}^\star(\vec\bsh_k, +1) - \hat Q_{\vec\lambda, K}^\star(\vec\bsh_k, -1)$. 
In view of Corollary \ref{cor:struc_of_iv-opt_dtr}, the IV-optimal DTR at stage $K$, $\pi^\star_K(\vec\bsh_k)$, can be estimated by $\hpiq_K(\vec\bsh_k) = \sgn(\hat\contr_{\vec\lambda, K}(\vec\bsh_k))$. 
Moreover, the weighted value function of $\pi^\star$ at stage $K$, $V^{\pi^\star}_{\vec\lambda, K}(\vec\bsh_k)$, can be estimated by $\hat V^{\star}_{\vec\lambda, K} = \hat Q^\star_{\vec \lambda, K}(\vec\bsh_k, \hpiq_K(\vec\bsh_k))$.

Now, assume for any stage $t\geq k+1$, the specification of the IV-constrained sets \eqref{eq:IV_contrained_set_general} has been made, 
and the weighted value function at stage $t$, $V^{\pi^\star}_{\vec\lambda, t}(\vec\bsh_t)$, has been estimated by $\hat V^\star_{\vec\lambda, t}(\vec\bsh_t)$. 
In addition, assume that $R_t \in [\underline{C}_t, \overline{C}_t]$ almost surely (with respect to $p^\star_{a_k}(\cdot, \cdot|\vec\bsh_k)$).
At stage $k$, define the pseudo-outcome $PO_k(r_k, \bsx_{k+1}|\vec\bsh_k, a_k) = r_k + V^{\pi^\star}_{\vec\lambda, k+1}(\vec\bsh_k, a_k, r_k, \bsx_{k+1})$.
By construction, we have $PO_k(R_k, \bsX_{k+1}|\vec\bsh_k, a_k) \in [\sum_{t\geq k}\underline{C}_t, \sum_{t\geq k} \overline{C}_t]$ almost surely for $(R_k, \bsX_{k+1}) \sim p^\star_{a_k}(\cdot, \cdot|\vec\bsh_k)$. 
Thus, we can apply Manski-Pepper bounds again to bound the expected value of $PO_k(R_k, \bsX_{k+1}|\vec\bsh_k, a_k)$, and obtain an estimate $\hat Q_{\vec\lambda, k}^\star$ of the weighted $Q$-function of $\pi^\star$ at stage $k$; see Supplementary Materials \textcolor{red}{X} for detailed expressions. One nuance is that the pseudo-outcome $PO_k(r_k, \bsx_{k+1}|\vec\bsh_k, a_k)$ depends on the unknown quantity $V^{\pi^\star}_{\vec\lambda, k+1}$. At stage $k$, we have already obtained an estimate $\hat V^{\star}_{\vec\lambda, k+1}$ of $V^{\pi^\star}_{\vec\lambda, k+1}$. 
Thus, the pseudo-outcome can be estimated by $\hat{PO}_k(r_k, \bsx_{k+1}|\vec\bsh_k, a_k) = r_k + \hat V^{\star}_{\vec\lambda, k+1}(\vec\bsh_k, a_k ,r_k, \bsx_{k+1})$.

Finally, the contrast function $\contr_{\vec\lambda, k}^{\pi^\star}(\vec\bsh_k)$ is estimated by $\hat \contr^\star_{\vec\lambda, k}(\vec\bsh_k) = \hat Q_{\vec\lambda, k}^\star(\vec\bsh_k, +1) - \hat Q_{\vec\lambda, k}^\star(\vec\bsh_k, -1)$,
the IV-optimal DTR at stage $k$ is estimated by $\hpiq_k(\vec\bsh_k) = \sgn(\hat\contr_{\vec\lambda, k}(\vec\bsh_k))$,
and the weighted value function of $\pi^\star$ at stage $k$ is estimated by $\hat V^{\star}_{\vec\lambda, k} = \hat Q_{\vec \lambda, k}(\vec\bsh_k, \hpiq_k(\vec\bsh_k))$. In this way, we recursively estimate all the contrast functions and obtain an estimated IV-optimal DTR $\hpiq$.


\iffalse
More explicitly, analogous to \eqref{eq:mp_bound_psi}, let us define
\begin{align*}
% \begin{split}
    \psi_{k}(\vec{\bsh}_k, a_k, z_k; C)  & = C \cdot \bbP(A_k^\obs = -a_k \mid Z_k = z_k, \vec{\bsH}_k^\obs = \vec\bsh_k) \nonumber \\
    &\qquad + \mathbb{E}[PO_k(R^\obs_k, \bsX_{k+1}^\obs|\vec\bsh_k, a_k) \mid \vec{\bsH}_k^\obs = \vec\bsh_k, Z_k = z_k, A_k^\obs = a_k] \\
    \label{eq:mp_bound_psi_k}
    & \qquad \qquad\qquad\qquad
    \times \bbP(A_k^\obs = a_k \mid \vec{\bsH}_k^\obs = \vec\bsh_k, Z_k = z_k)\numberthis.
    % & \qquad + C \cdot \bbP(A_K^\obs = -a_k \mid Z_K = z_k, \vec{\bsH}_K^\obs = \vec\bsh_k)
% \end{split}
\end{align*}
Manski-Pepper bounds give that $\bbE_{(R_k, \bsX_{k+1}) \sim p^\star_{a_k}(\cdot, \cdot|\vec\bsh_k)}[PO_k(R_k, \bsX_{k+1}|\vec\bsh_k, a_k)]$ can be lower and upper bounded by 
\begin{align*}
    & \bbP(Z_k = -1 |\vec{\bsH}_k^\obs= \vec\bsh_k) \cdot \psi_{k}\bigg(\vec{\bsh}_k, a_k, -1; \sum_{t\geq k}\underline{C}_t\bigg) \\
    \label{eq:mp_lower_bound_k}
    & ~~+ \bbP(Z_k = +1 |\vec{\bsH}_k^\obs = \vec\bsh_k)\cdot 
    \bigg[\psi_{k}\bigg(\vec{\bsh}_k, a_k, -1; \sum_{t\geq k}\underline{C}_t\bigg)
    \lor
    \psi_{k}\bigg(\vec{\bsh}_k, a_k, +1; \sum_{t\geq k}\underline{C}_t\bigg)\bigg]\numberthis\\
    \text{and}& \\
    & \bbP(Z_k = -1 |\vec{\bsH}_k^\obs = \vec\bsh_k) 
    \cdot 
    \bigg[ 
    \psi_{k}\bigg(\vec{\bsh}_k;, a_k, -1; \sum_{t\geq k}\overline{C}_t \bigg)
    \land 
    \psi_{k}\bigg(\vec{\bsh}_k, a_k, +1; \sum_{t\geq k}\overline{C}_k \bigg)\bigg]\\
    % & \bbP(Z_K = -1 |\vec{\bsH}_K^\obs= \vec\bsh_k) \cdot \psi_{K}(\vec{\bsh}_K, a_K, -1; \underline{C}_K) \\
    \label{eq:mp_upper_bound_k}
    & ~~ + \bbP(Z_k = +1|\vec{\bsH}_k^\obs = \vec\bsh_k)\cdot \psi_{k}\bigg(\vec\bsh_k, a_k, +1 ; \sum_{t\geq k}\overline{C}_t \bigg),\numberthis
\end{align*}
respectively.

Similar to the situation at the final stage, as long as we take $\calF_k\supseteq \{PO_k(\cdot, \cdot|\vec\bsh_k, a_k)\}$ when defining $\calP_{\vec\bsh_k, a_k}$ in \eqref{eq:IV_contrained_set_general}, then the worst-case and best-case $Q$ functions at stage $k$ defined in \eqref{eq:worst_Q_func_k}--\eqref{eq:best_Q_func_k} can be set to \eqref{eq:mp_lower_bound_k} and \eqref{eq:mp_upper_bound_k}, respectively. Along with the specification of $\lambda_k(\vec\bsh_k, a_k)$, we finish the construction of the weighted $Q$-function $Q_{\vec\lambda, k}(\vec\bsh_k, a_k)$ at stage $k$.


The only obstruction in estimating $Q_{\vec\lambda, k}(\vec\bsh_k, a_k)$ is that in the definition of $\psi_k$, the pseudo-outcome $PO_k(r_k, \bsx_{k+1}|\vec\bsh_k, a_k) = r_k + V^{\pi^\star}_{\vec\lambda, k+1}(\vec\bsh_k, a_k, r_k ,\bsx_{k+1})$ depends on the unknown quantity $\pi^\star$. 
Luckily, at stage $k$, we have already obtained an estimate $\hat V^{\star}_{\vec\lambda, k+1}$ of $V^{\pi^\star}_{\vec\lambda, k+1}$. 
Thus, we can estimate the pseudo-outcome by $\hat{PO}_k(r_k, \bsx_{k+1}|\vec\bsh_k, a_k) = r_k + \hat V^{\star}_{\vec\lambda, k+1}(\vec\bsh_k, a_k ,r_k, \bsx_{k+1})$. Replacing $PO_k$ by its estimated version, the function $\psi_k$ defined in \eqref{eq:mp_bound_psi_k}, and thus the quantities defined in \eqref{eq:mp_lower_bound_k} and \eqref{eq:mp_upper_bound_k}, are now completely identified from the observed data distribution. 
As the result, we can obtain an estimate $\hat Q_{\vec\lambda, k}^\star$ of the weighted $Q$-function at stage $k$. 
\fi









% \begin{equation}
%     \begin{split}
%     \underline{\Qfunc}_{K}(\vec\bsh_k, a_K) &= P(Z_K = -1 |\vec{\bsh}_K) \cdot \psi_{-1, a_K}(R_K, \vec{\bsh}_K; \underline{C}_K) \\
%     &+ P(Z_K = +1 |\vec{\bsh}_K)\cdot \max\{\psi_{-1, a_K}(R_K, \vec{\bsh}_K; \underline{C}_K), \psi_{+1, a_K}(R_K, \vec{\bsh}_K; \underline{C}_K)\},\\
%      \overline{\Qfunc}_{K}(\vec\bsh_k, a_K) &= 
%      P(Z_K = -1 |\vec{\bsh}_K) \cdot \min\{\psi_{-1, a_K}(R_K, \vec{\bsh}_K; \overline{C}_K ), \psi_{+1, a_K}(R_K, \vec{\bsh}_K; \overline{C}_K )\}\\
%     &+ P(Z_K = +1|\vec{\bsh}_K)\cdot \psi_{+1, a_K}(R_K, \vec{\bsh}_K; \overline{C}_K ), ~a_K = \pm 1.
%     \end{split}
% \end{equation}
% In practice, we estimate each component in $\psi_{Z_K = z, A_K = a}(R_K, \vec{\bsh}_K; C)$ using parametric models or flexible machine learning tools like regression tress, replace each quantity with its estimated analogue, and obtain $\big\{\widehat{\underline{\Qfunc}}_{K, i}(\vec\bsh_{K, i}, \pm 1), \widehat{\overline{\Qfunc}}_{K, i}(\vec\bsh_{K, i}, \pm 1),~i = 1, 2, \cdots, n\big\}$. 
% Next, for pre-specified $\lambda_K(\vec\bsh_k, \pm 1)$, we calculate $\widehat{\Qfunc}_{\vec{\lambda}, K, i}(\vec\bsh_{K, i}, \pm 1)$ according to \eqref{eq:wted_Q_func_K}, and estimate the $K$-th stage decision rule $\pi^\star_K$ in some pre-specified function class via solving the weighted classification problem \eqref{eq:classification DTR}. See Remark \ref{remark: DTR choose lambda} for choices of $\lambda_K(\vec\bsh_k, \pm 1)$ suited for different purposes. Lastly, $\Vfunc_{\vec{\lambda}, K, i}^{\pi^\star}(\vec\bsh_{K, i})$ is estimated by $\widehat{\Vfunc}_{\vec{\lambda}, K, i}^{\widehat{\pi}^\star}(\vec\bsh_{K, i}) = \widehat{\Qfunc}_{\vec{\lambda}, K, i}\big(\vec\bsh_{K, i}, ~\sgn\big\{\widehat{Q}_{\vec{\lambda}, K, i}(\vec\bsh_{K, i}, +1) - \widehat{Q}_{\vec{\lambda}, K, i}(\vec\bsh_{K, i}, -1)\big\}\big)$.


% \newpage

% Next, at stage $K - 1$, define a pseudo-outcome $PO_{K - 1, i} = R_{K - 1, i} + \widehat{\Vfunc}_{\vec{\lambda}, K, i}^{\widehat{\pi}^\star}(\vec\bsh_{K, i})$ for each unit. Assume $R_{K - 1} \in [C^{K-1}_0, C^{K-1}_1]$ with probability $1$ so that $PO_{K-1} \in [\textcolor{red}{XX, XX}]$ with probability $1$. Define 
% \begin{equation}
% \begin{split}
%     &\psi_{Z_{K-1} = z, A_{K-1} = a}(PO_{K-1}, \vec{\bsh}_{K-1}; C) \\
%     = ~&\mathbb{E}\{PO_{K-1} \mid Z_{K-1} = z, A_{K-1} = a, \vec{\bsh}_{K-1}\}\cdot P(A_{K-1} = a \mid Z_{K-1} = z, \vec{\bsh}_{K-1})\\ 
%     &+C \cdot P(A_{K-1} = -a \mid Z_{K-1} = z, \vec{\bsh}_{K-1}).
% \end{split}
% \end{equation}
% For some pre-specified choice of  $\lambda_{K-1}(\vec\bsh_{K-1}, \pm 1)$, we then obtain estimates $\widehat{\underline\Qfunc}^\pi_{\vec{\lambda}, K-1, i}(\vec\bsh_{K-1, i}, \pm 1)$, $\widehat{\overline\Qfunc}^\pi_{\vec{\lambda}, K-1, i}(\vec\bsh_{K-1, i}, \pm 1)$, $\widehat{\Qfunc}_{\vec{\lambda}, K-1, i}(\vec\bsh_{K-1, i}, \pm 1)$, and $\widehat{\Vfunc}_{\vec{\lambda}, K-1, i}^{\widehat{\pi}^\star}(\vec\bsh_{K-1, i})$ for $i = 1, 2, \cdots, n$
% as in the $K$-th stage and estimate $\pi^\star_{K-1}$ by solving a second weighted classification problem. The procedure then carries onwards. Algorithm \ref{alg} summarizes the estimation procedure.





\begin{algorithm}[t!] 
\SetAlgoLined
\caption{Estimation of the IV-Optimal DTR} \label{alg}
\vspace*{0.12 cm}
\KwIn{Trajectories and instrument variables $\{(\bsx_{k, i}, a_{k, i}, r_{k, i}, z_{k, i}): k \in[K], i\in[n]\}$, weighting functions $\{\lambda(\vec\bsh_k, a_k)\}$, policy class $\Pi$, forms of partial identification intervals.}%, a sequence of constants $\{\lambda_k(\vec\bsh_{k}, a_k), ~1 \leq k \leq K\}$, \text{and} IV identification assumptions;}
\KwOut{Estimated IV-optimal DTR $\hat\pi^\star$.}
\texttt{{\# Stage \RN{1}: Q-learning}} \\
% Construct $\underline{Q}_K, \overline{Q}_K$ and estimate them by $\hat{\underline{Q}}_K, \hat{\overline{Q}}_K$ using $\{\vec\bsh_{K, i}\}_{i=1}^n$\;
Obtain an estimate $\hat Q^\star_{\vec\lambda, K}$ of $Q_{\vec\lambda, K}$ using using $(\vec\bsh_{K, i}, r_{K, i}, z_{K, i})_{i=1}^n$\;
Estimate $\contr_{\vec\lambda, K}$ by $\hat \contr^\star_{\vec\lambda, K}(\vec\bsh_K) = \hat Q_{\vec\lambda, K}^\star(\vec\bsh_K, +1) - \hat Q_{\vec\lambda, K}^\star(\vec\bsh_K, -1)$\;
Set $\hpiq_K(\vec\bsh_K) = \sgn(\hat \contr^\star_{\vec\lambda, K}(\vec\bsh_K))$ and $\hat V^\star_{\vec\lambda, k}(\vec\bsh_K) = \hat Q_{\vec\lambda, K}^\star(\vec\bsh_K, \hpiq_K(\vec\bsh_K))$\;
\For{$k = K-1, \hdots, 1$}{
  For each $i\in[n]$, construct $\hat{PO}_{k, i} = r_{k, i} + \hat V^{\star}_{\vec\lambda, k+1}(\vec\bsh_{k+1, i})$\;
  Obtain an estimate $\hat Q^\star_{\vec\lambda, k}$ of $Q_{\vec\lambda, k}^{\pi^\star}$ using using $(\vec\bsh_{k, i}, \hat{PO}_{k, i}, z_{k, i})_{i=1}^n$\;
  % Construct $\underline Q_{\vec\lambda, k}^{\pi^\star}, \overline Q_{\vec\lambda, k}^{\pi^\star}$ and estimate them by $\hat{\underline Q}_{\vec\lambda, k}^{\star}, \hat{\overline Q}_{\vec\lambda, k}^{\star}$
  Estimate $\contr_{\vec\lambda, k}^{\pi^\star}$ by $\hat \contr^\star_{\vec\lambda, k}(\vec\bsh_k) = \hat Q_{\vec\lambda, k}^\star(\vec\bsh_k, +1) - \hat Q_{\vec\lambda, K}^\star(\vec\bsh_k, -1)$\;
  Set $\hpiq_k(\vec\bsh_k) = \sgn(\hat \contr^\star_{\vec\lambda, k}(\vec\bsh_k))$ and $\hat V^\star_{\vec\lambda, k}(\vec\bsh_k) = \hat Q_{\vec\lambda, k}^\star(\vec\bsh_k, \hpiq_k(\vec\bsh_k))$\;
  
}
\texttt{{\# Stage \RN{2}: Weighted classification}} \\
\For{$k = K, \hdots, 1$}{
  Solve the weighted classification problem in \eqref{eq:wted_classification_dtr} to obtain $\hat\pi^\star_k$\;
}
\Return{$\hat \pi^\star$}
\label{alg:IV-optimal_DTR}
\end{algorithm}


\paragraph{Obtaining parsimonious policies via weighted classification.}
In many applications, it is desirable to impose additional constrains on the estimated DTR. For example, one may require the DTR to be parsimonious and thus more interpretable. Such constraints are usually encoded by a restricted function class $\Pi = \Pi_1 \times \cdots \times \Pi_K$, such that any $\pi\notin \Pi$ will not be considered. 

We next introduce a strategy that ``projects'' $\hpiq$, the DTR obtained by $Q$-learning and is thus not necessarily inside $\Pi$, onto the function class $\Pi$. Recall the formula for the IV-optimal DTR $\pi^\star$ given in \eqref{eq:struc_of_iv-opt_dtr}. With some algebra, one readily checks that $\pi^\star$ is a solution to the following weighted classification problem:
\begin{equation}
  \label{eq:wted_classification_dtr}
  \pi^\star_k(\vec\bsh_k) \in \argmin_{a_k\in\{\pm 1\}} |\contr^{\pi^\star}_{\vec\lambda, k}(\vec\bsh_{k})| \cdot \indc{\sgn(\contr^{\pi^\star}_{\vec\lambda, k}(\vec\bsh_{k})) \neq a_k}.
\end{equation}






The above representation %\eqref{eq:wted_classification_dtr}
% Theorem \ref{thm:struc_of_iv-opt_dtr} 
illuminates a rich class of strategies to search for a DTR $\pi$ within a desired, possibly parsimonious function class $\Pi$, via sequentially solving the following weighted classification problem:
\begin{equation}
  \hat \pi^\star_k(\vec\bsh_k) \in \argmin_{\pi_k \in \Pi_k} \frac{1}{n}\sum_{i=1}^n |\hat\contr^\star_{\vec\lambda, k}(\vec\bsh_{k, i})| \cdot \indc{\sgn(\hat\contr^\star_{\vec\lambda, k}(\vec\bsh_{k, i})) \neq \pi_k(\vec\bsh_{k, i})},
\end{equation}
where we recall that $\hat\contr^\star_{\vec\lambda, k}$ is an estimate of $\hat\contr^{\pi^\star}_{\vec\lambda, k}$ obtained via $Q$-learning, and $\{\vec\bsh_{k, i}\}_{i=1}^n$ is the historical information at stage $k$ in our dataset. This strategy bears similarities with the strategy proposed in \citet{zhao2015new}. The estimation procedure is summarized in Algorithm \ref{alg:IV-optimal_DTR}.

%\begin{lemma}\label{lemma: DTR classification}
%The regime at stage $k$ constructed in Theorem \ref{thm:struc_of_iv-opt_dtr} is equivalent to
%\begin{equation}
%\label{eq:classification DTR}
%    \pi^\star_k = \argmin_{\pi_k} \bigg|Q_{\vec{\lambda}, k}^{\pi^\star}(\vec\bsh_k, +1) - Q_{\vec{\lambda}, k}^{\pi^\star}(\vec\bsh_k, -1)\bigg| \cdot \Indc\bigg\{\sgn\bigg(Q_{\vec{\lambda}, k}^{\pi^\star}(\vec\bsh_k, +1) - Q_{\vec{\lambda}, k}^{\pi^\star}(\vec\bsh_k, -1)\bigg) \neq \pi_k(\vec\bsh_k)\bigg\}.
%\end{equation}
%\end{lemma}
%Lemma \ref{lemma: DTR classification} allows researchers to recast the problem of estimating $\pi_k^\star(\vec{\bsh}_k)$ at stage $k$ into a weighted classification problem and search for a treatment rule within a desired, possibly parsimonious function class. Let $\widehat{\pi}_{k+1}^\star$ be an estimate of $\pi^\star_{k+1}$ at stage $k+1$, and $\widehat{Q}_{\vec{\lambda}, k, i}^{\widehat{\pi}^\star}(\vec\bsh_{k, i}, \pm 1)$ estimates of $Q_{\vec{\lambda}, k, i}^{\pi^\star}(\vec\bsh_{k, i}, \pm 1)$ for $i = 1, 2, \cdots, n$, then $\pi^\star_k$ at stage $k$ can be estimated via solving the following empirical analogue of \eqref{eq:classification DTR} within a desired function class $\Pi_k$:
% \begin{equation}\small
% \label{eq: classification DTR}
%     \widehat{\pi}^\star_k = \argmin_{\pi_k \in \Pi_k} \sum_{i = 1}^n  \bigg|\widehat{Q}_{\vec{\lambda}, k, i}^{\widehat{\pi}^\star}(\vec\bsh_{k, i}, +1) - \widehat{Q}_{\vec{\lambda}, k, i}^{\widehat{\pi}^\star}(\vec\bsh_{k, i}, -1)\bigg| \cdot \Indc\bigg\{\sgn\left\{\widehat{Q}_{\vec{\lambda}, k, i}^{\widehat{\pi}^\star}(\vec\bsh_{k, i}, +1) - \widehat{Q}_{\vec{\lambda}, k, i}^{\widehat{\pi}^\star}(\vec\bsh_{k, i}, -1)\right\} \neq \pi_k(\vec\bsh_{k, i})\bigg\},
% \end{equation}
% where $\widehat{Q}_{\vec{\lambda}, k, i}^{\widehat{\pi}^\star}(\vec\bsh_{k, i}, \pm 1)$ are estimates of $Q_{\vec{\lambda}, k, i}^{\pi^\star}(\vec\bsh_{k, i}, \pm 1)$ for $i = 1, 2, \cdots, n$.














==> old_tex/0402-dtr.tex <==
%!TEX root = main.tex
\section{Improving Dynamic Treatment Regimes with an Instrumental Variable}\label{sec:dtr_improve}

In this section, we show how the IV-optimality framework developed in Section \ref{sec: extension to DTR} can be modified to tackle the policy improvement problem under the multiple-stage setup.
Let $\pibase$ be a baseline DTR that we aim to improve upon. 
Some most important baseline DTRs include the standard-of-care DTR (i.e., $\pibase_k = -1$ for any $k$) and the SRA-optimal DTR defined in Section \ref{subsec: DTR setup}. 
The goal of policy improvement, as discussed in Section \ref{sec: ITR IV improve}, is to obtain a DTR $\piimp$ so that $\pibase$ is no worse and potentially better than $\pibase$.
% In this section, we explore leveraging additional IV information to construct an improved regime $\piimp$ such that it can do \emph{no worse} and potentially improve upon $\pibase$. 

To achieve this goal, we leverage the IV information, encoded in the collection of IV-constrained sets $\{\calP_{\vec\bsh_k, a_k}\}$. 
We are to introduce the notion of \emph{IV-improved DTR}, generalizing the notion of IV-improved ITR appeared in Definitions \ref{def:risk_based_improvement} and \ref{def:value_based_improvement}.
To start with, let us define the following {relative $Q$-functions} and the corresponding {relative value functions} of a DTR $\pi$ with respect to the baseline DTR $\pibase$.

\begin{definition}[Relative $Q$-function and value function]
The {relative $Q$-function} of a DTR $\pi$ with respect to the baseline DTR $\pibase$ at stage $K$ is
\begin{align}
  \label{eq:rel_Q_func_K}
  &\Qfunc^{\pi\rel\pibase}_K (\vec\bsh_K, a_K)
  = \inf_{ \substack{
  p_{a_K}\in\calP_{\vec\bsh_K, a_K}
  \\ p_{a_K'}\in\calP_{\vec\bsh_K, a_K'} }
  }
  \bigg\{\bbE_{\substack{R_K\sim p_{a_K} \\ R_K'\sim p_{a_K'}}} \left[R_K - R_K'\right] \bigg\}
  % ,
  % \Vfunc^{\pi\rel\pibase}_K(\vec\bsh_K) = \Qfunc^{\pi\rel\pibase}_K \big(\vec\bsh_K, \pi_K(\vec\bsh_K)\big)
  ,
\end{align}
where $a_K' = \pibase_K(\vec\bsh_k)$ is the action taken according to the baseline DTR. The corresponding relative value function is defined as $\Vfunc^{\pi\rel\pibase}_K(\vec\bsh_K) = \Qfunc^{\pi\rel\pibase}_K \big(\vec\bsh_K, \pi_K(\vec\bsh_K)\big)$. 
Recursively, at stage $k = K - 1, K - 2, \cdots, 1$, the relative $Q$-function of $\pi$ with respect to $\pibase$ is defined as
\begin{align}
  \label{eq:rel_Q_func_k}
  Q^{\pi\rel\pibase}_k(\vec\bsh_k, a_k)
  & = 
  \inf_{ \substack{
  p_{a_k}\in\calP_{\vec\bsh_k, a_k}
  \\ p_{a_k'}\in\calP_{\vec\bsh_k, a_k'} }
  }
  \bigg\{
  \bbE_{\substack{(R_k, \bsX_{k+1})\sim p_{a_k} \\ (R_k', \bsX'_{k+1})\sim p_{a_k'} }} 
  \big[R_k - R_k' + \Vfunc_{k+1}^{\pi\rel\pibase}(\vec\bsH_{k+1})\big]
  \bigg\},
\end{align}
where $a_k' = \pibase_k(\vec\bsh_k)$ and $\vec\bsH_{k+1} = (\vec\bsh_k, a_k, R_k, \bsX_{k+1})$.
The corresponding relative value function is $\Vfunc^{\pi\rel\pibase_k}_k(\vec\bsh_k) = \Qfunc^{\pi\rel\pibase}_{k}\big(\vec\bsh_k, \pi_k(\vec\bsh_k)\big)$.
\end{definition}

The relative value function $V^{\pi\rel\pibase}_k$ at stage $k$ captures the cumulative worst-case (subject to the IV constraints) excess value of following the DTR $\pi$ over $\pibase$ from stage $k$ and onwards.
Note that the relative value function $V^{\pi\rel\pibase}_K$ at stage $K$ is analogous to the objective function in \eqref{eq:PIO_value}.
Maximizing the relative value functions would then deliver a DTR that follows the baseline regime $\pibase$ unless there is compelling evidence not to, similar to the IV-improved ITR whose explicit form is given in Propositions \ref{prop:itr_policy_imp_bayes_policy_classification} and \ref{prop:itr_policy_imp_bayes_policy_value}.

We are now ready to define the estimand of interest, generalizing Definitions \ref{def:risk_based_improvement} and \ref{def:value_based_improvement}. 

\begin{definition}[IV-improved DTR]\label{def:DTR imp operator}
Let $\pibase$ be a baseline DTR, $\Pi$ a policy class, and $\{\calP_{\vec\bsh_k, a_k}\}$ a collection of IV-constrained sets. 
% A DTR improvement operator, denoted as $\mathcal{IP}^{\textsf{D}}$, refers to an operator that maps $\pibase$ to a regime $\piimp$ such that the relative value of $\pi$ with respect to $\pibase$ at stage $1$ is maximized, i.e.,
A DTR $\piimp$ is said to be IV-improved if it satisfies
\begin{equation}
\label{eq:dtr_imp_optimization}
 \piimp \in \argmax_{\pi\in \Pi} V^{\pi\rel\pibase}_1(\bsx_1)
\end{equation}
for every fixed $\bsh_1 = \bsx_1 \in \calX$.
\end{definition}

Analogous to Theorem \ref{thm:iv_opt_dtr_dynamic_prog}, the following result solves the optimization problem \eqref{eq:dtr_imp_optimization} using a dynamic programming approach when $\Pi$ is the collection of all DTRs.
\begin{theorem}[Dynamic Programming for DTR Improvement Operator]
  \label{thm:iv_imp_dtr_dynamic_prog}
Let $\piimp$ be recursively defined as follows:
\begin{align}
  \label{eq:iv_imp_dtr_dynamic_prog_expression}
  \piimp_K(\vec\bsh_K) & = \argmax_{a_K\in\{\pm 1\}} \Qfunc_{K}^{\piimp\rel\pibase}(\vec\bsh_K, a_K), %\\
  ~~\piimp_k(\vec\bsh_k) = \argmax_{a_k\in\{\pm 1\}} \Qfunc^{\piimp\rel\pibase}_{k}(\vec\bsh_k, a_k), ~k = K-1, \hdots, 1.
\end{align}
Then the DTR $\piimp$ satisfies
\begin{equation}
  \label{eq:iv_imp_dtr_k}
  V^{\piimp\rel\pibase}_{k}(\vec\bsh_k) = \max_{\pi} V^{\pi\rel\pibase}_{k}(\vec\bsh_k)
\end{equation}
for any stage $k$ and any configuration of the historical information $\vec\bsh_k$, where the maximization is taken over all DTRs.
\end{theorem}

The following corollary is similar to Corollary \ref{cor:struc_of_iv-opt_dtr}, and gives an alternative characterization of the IV-improved DTR.

\begin{corollary}[Alternative characterization of the IV-improved DTR]
\label{cor:struc_of_iv-imp_dtr}
Recursively define $\piimp$ as
\begin{equation}
  \label{eq:struc_of_iv-imp_dtr}
  \piimp_k(\vec\bsh_k) = \pibase_k(\vec\bsh_k)
   \cdot 
   \sgn\big\{\contr^{\piimp\rel\pibase}_k(\vec\bsh_k) \big\}
   % \sgn\big(L_{\lambda, k}^{\pi^\star}(\vec\bsH_k) +U_{\lambda, k}^{\pi^\star}(\vec\bsH_k) \big)
   , ~~ k = K, \hdots, 1,
\end{equation}  
where for $a_{k}' = \pibase_k(\vec\bsh_k), \vec\bsH_{k+1} = (\vec\bsh_k, a_k, R_k, \bsX_{k+1})$ and $\vec\bsH_{k+1}' = (\vec\bsh_k, a_k', R_k', \bsX_{k+1}')$, the quantities
\begin{align}
  \contr^{\piimp\rel\pibase}_K(\vec\bsh_K) & =  
  \sup_{p_{a_K'}\in \calP_{\vec\bsh_K, a_K'}} 
  \bbE_{R_K'\sim p_{a_K'}}
  [R_K'] 
  - 
  \inf_{p_{-a_K'}\in \calP_{\vec\bsh_K, -a_K'}} 
  \bbE_{R_K\sim p_{-a_K'} }
  [ R_K  ], ~\text{and} 
  \nonumber \\
  \contr^{\piimp\rel\pibase}_k(\vec\bsh_k) & = 
  \sup_{p_{a_k'}\in \calP_{\vec\bsh_k, a_k'}} 
  \bbE_{(R_k', \bsX_{k+1}')\sim p_{a_k'}}
  [R_k'] 
  +
  \inf_{p_{a_k'}\in \calP_{\vec\bsh_k, a_k'}}
  \bbE_{(R_k', \bsX_{k+1}') \sim p_{a_k'}}[V^{\piimp\rel\pibase}_k(\vec\bsH_{k+1}')]
  \nonumber \\
  \label{eq:iv-imp_cate}
  & \qquad - 
  \inf_{p_{-a_k'}\in \calP_{\vec\bsh_k, -a_k'}} 
  \bbE_{(R_k, \bsX_{k+1})\sim p_{-a_k'} }
  [ R_k + V^{\piimp\rel\pibase}_{k+1}(\vec\bsH_{k+1}) ] 
  , ~ 1 \leq k \leq K-1,
\end{align}
depend on $\piimp$ only through $\piimp_{(k+1):K}$ and are therefore well-defined.
Then $\piimp$ satisfies \eqref{eq:iv_imp_dtr_k} for any stage $k$ and any configuration of the historical information $\vec\bsh_k$.
In particular, 
$\piimp$ is an IV-improved DTR in the sense of Definition \ref{def:DTR imp operator} when $\Pi$ is the set of all DTRs.
\end{corollary}

While the expressions in \eqref{eq:iv_imp_dtr_k} and \eqref{eq:iv-imp_cate} look complicated, they actually admit a rather intuitive explanation. The contrast function $\contr^{\piimp\rel\pibase}_k$ measures the cumulative worst-case gain of following $\piimp$ over $\pibase$, starting from stage $k$, and one would only flip the decision made by $\pibase_k$ if this worse-case gain is positive. In fact, with some algebra, one readily checks that $\piimp_K$ can be expressed in a similar form as \eqref{eq: bayes rule} and \eqref{eq: bayes rule II}. 
% The expressions for $\piimp_k$ is more complicated when $k\leq K-1$.

Given Corollary \ref{cor:struc_of_iv-imp_dtr}, the strategy in Section \ref{subsec: estimate IV-optimal DTR}, and in particular Algorithm \ref{alg:IV-optimal_DTR}, can be modified in a \emph{mutatis mutandis} fashion to give an algorithm for estimating the IV-improved DTR. For brevity, we refer the readers to Supplementary Material \textcolor{red}{X} for details.

% In practice, researchers may recast the problem of searching for $\piimp_k$ in a pre-specified function class $\Pi_k$ into a classification problem again; we defer details to the Supplementary Material XX. 
















==> old_tex/05-example.tex <==
\section{An Illustrative Example: Two-Stage Sequential Randomized Trial with Noncompliance}
\label{sec: illustrate two-stage example}
To further illustrate the framework and the proposed method, we consider a simple, two-stage sequential randomized controlled trial with noncompliance. We generate time-independent baseline covariates $X_1, X_2 \sim \text{Normal}(0, 1)$. At stage $1$, a treatment $Z_1$ is randomly assigned. We use $Z_1 = +1$ to denote assigning the treatment and $Z_1 = -1$ to denote not assigning the treatment. Subjects receiving the treatment assignment may not comply with the assignment and hence induces noncompliance. In practice, subjects' noncompliance is likely to be due to some unmeasured confounding variables, e.g., motivation in a smoking cessation trial. The actual treatment received $A_1$, the unmeasured confounder $U_1$, and the stage-$1$ reward follow the following data-generating process:

\begin{equation}
\begin{split}
    &Z_1 = \begin{cases} +1,~\text{w.p.}~0.5,\\
    -1,~\text{w.p.}~0.5,\\
    \end{cases}
    \quad U_1 \sim \text{Bernoulli}(1/2),\quad A_1 \mid Z_1, X_1, X_2, U_1 =\begin{cases}
    +1,~\text{w.p.}~\text{expit}\{Z_1 + U_1\},\\
    -1,~\text{w.p.}~1-\text{expit}\{Z_1 + U_1\},\\
    \end{cases} \\
    &R_1 \mid X_1, X_2, U_1, A_1 \sim \text{Normal}(0.2U_1 + 0.3X_1A_1, 1)~\text{truncated at} -1.5~\text{and}~1.5.
\end{split}
\end{equation}
We then specify a similar data-generating process at the second stage. Note that according to the DGP, the stage-$1$ treatment received $A_1$ has a direct effect on the stage-$2$ reward $R_2$, and the stage-$1$ reward $R_1$ is an effect modifier of the stage-$2$ effect. By the study design, randomly assigned treatments $Z_1$ and $Z_2$ are valid instrumental variables.

\begin{equation}
\begin{split}
    &Z_2 = \begin{cases} +1,~\text{w.p.}~0.5,\\
    -1,~\text{w.p.}~0.5,\\
    \end{cases}
    \quad U_2 \sim \text{Bernoulli}(1/2),\\
    &A_2 \mid X_1, X_2, Z_2, U_2, R_1 =\begin{cases}
    +1,~\text{w.p.}~\text{expit}\{Z_2 + 0.5R_1 - 0.5U_2\},\\
    -1,~\text{w.p.}~1-\text{expit}\{Z_2 + 0.5R1 - 0.5U_2\},\\
    \end{cases} \\
    &R_2 \mid X_1, X_2, U_2, R_1, A_1, A_2 \sim \text{Normal}(0.2U_2 + 0.2X_1A_1 + 0.2(0.5R_1 - U_2)A_2, 1)~ \text{truncated at} -2~\text{and}~2.
\end{split}
\end{equation}

\begin{figure}
    \centering
 \begin{tikzpicture}[
every text node part/.style={align=center},
squarednode/.style={rectangle, draw=black, fill=white, very thick, minimum size=5mm}
]
%Nodes Stage 2
\node at (-1, 4) {Stage 2:};
\node[squarednode, draw = black, fill = white] at (2,4)  (1_R1) {$R_1 < 0.65$};
\node[squarednode, draw = red] at (0, 2) (1_R1_yes) {Assign \\ $A_2 = -1$};
%\node[squarednode] at (0, 2) (1_R1_yes) {$R_1 \geq -1.3$};
\node[squarednode, draw = red] at (4, 2) (1_R1_no) {Assign \\ $A_2 = +1$};
%\node[squarednode, draw = red] at (-2, 0) (1_R1_yes_yes) {Assign \\ $A_2 = -1$};
%\node[squarednode, draw = red] at (2, 0) (1_R1_yes_no) {Assign \\ $A_2 = +1$};

%Nodes Stage 1
\node at (7, 4) {Stage 1:};
\node[squarednode, draw = black, fill = white] at (10, 4)  (1_X1) {$X_1 < -0.53$};
\node[squarednode, draw = red] at (8, 2) (1_X1_yes) {Assign \\ $A_2 = -1$};
\node[squarednode, draw = red] at (12, 2) (1_X1_no) {Assign \\ $A_2 = +1$};

%Lines Stage 2
\draw[ultra thick, ->] (1_R1) -- (1_R1_yes);
\draw[ultra thick, ->] (1_R1) -- (1_R1_no);
%\draw[ultra thick, ->] (1_R1_yes) -- (1_R1_yes_yes);
%\draw[ultra thick, ->] (1_R1_yes) -- (1_R1_yes_no);

%Lines Stage 1
\draw[ultra thick, ->] (1_X1) -- (1_X1_yes);
\draw[ultra thick, ->] (1_X1) -- (1_X1_no);
\end{tikzpicture}%
\caption{An estimated IV-optimal two-stage dynamic treatment regime corresponding to letting $\lambda(\vec\bsH_2, \pm 1) = \lambda(\vec\bsH_1, \pm 1) = 1/2$.}
\label{fig: illustrate two-stage tree}
\end{figure}

\begin{figure}
    \centering
    \begin{tikzpicture}[every text node part/.style={align=center},
    node distance=2cm]
% nodes

% Stage 1
\draw[gray, ultra thick] (-2,0) -- (2,3);
\draw[gray, ultra thick] (-2,0) -- (2,-3);
\filldraw[black] (-2,0) circle (2pt);
\node at (-2.5, 0) {$\vec{\bsH_1}$};
\node[align=left] at (-0.2,2) {\small $a_1 = +1$};
\node[align=left] at (-0.2,-2) {\small $a_1 = -1$};
\draw[|-|, ultra thick] (2,2) -- (2,4);
\draw[|-|, ultra thick] (2,-2) -- (2,-4);

\node at (3.5, 4) {\small $\overline{\Qfunc}^{\pi^\ast}_{\vec{\boldsymbol\lambda}, 1} (\vec\bsH_1, +1) $};
\node at (3.5, 2) {\small $\underline{\Qfunc}^{\pi^\ast}_{\vec{\boldsymbol\lambda}, 1} (\vec\bsH_1, +1)  $};

\node at (3.5, -2) {\small $\overline{\Qfunc}^{\pi^\ast}_{\vec{\boldsymbol\lambda}, 1} (\vec\bsH_1, +1)  $};
\node at (3.5, -4) {\small $\underline{\Qfunc}^{\pi^\ast}_{\vec{\boldsymbol\lambda}, 1} (\vec\bsH_1, +1)  $};

% Stage 2
\draw[-, gray, ultra thick, dashed] (2, 3) -- (7, 3);
\draw[-, gray, ultra thick, dashed] (2, -3) -- (7, -3);

\filldraw[black] (7, 3) circle (2pt);
\node at (6.5, 3.5) {$\vec{\bsH_2}$};
\draw[gray, ultra thick] (7,3) -- (9.7,5);
\draw[gray, ultra thick] (7,3) -- (9.7,1);
\draw[|-|, ultra thick] (9.7,4.5) -- (9.7,5.5);
\draw[|-|, ultra thick] (9.7,0.5) -- (9.7,1.5);
\node[align=left] at (8,4.35) {\small $a_2 = +1$};
\node[align=left] at (8,1.65) {\small $a_2 = -1$};
\node at (11.2, 5.5) {\small$\overline{\Qfunc}_{\vec{\boldsymbol\lambda}, 2} (\vec\bsH_2, +1)$};
\node at (11.2, 4.5) {\small$\underline{\Qfunc}_{\vec{\boldsymbol\lambda}, 2} (\vec\bsH_2, +1)  $};
\node at (11.2, 1.5) {\small$\overline{\Qfunc}_{\vec{\boldsymbol\lambda}, 2} (\vec\bsH_2, -1)  $};
\node at (11.2, 0.5) {\small$\underline{\Qfunc}_{\vec{\boldsymbol\lambda}, 2} (\vec\bsH_2, -1)  $};

\filldraw[black] (7, -3) circle (2pt);
\node at (6.5, -3.5) {$\vec{\bsH'_2}$};
\draw[gray, ultra thick] (7,-3) -- (9.7,-5);
\draw[gray, ultra thick] (7,-3) -- (9.7,-1);
\draw[|-|, ultra thick] (9.7,-4.5) -- (9.7,-5.5);
\draw[|-|, ultra thick] (9.7,-0.5) -- (9.7,-1.5);
\node[align=left] at (8,-4.35) {\small $a_2 = -1$};
\node[align=left] at (8,-1.65) {\small $a_2 = +1$};
\node at (11.2, -4.5) {\small$\overline{\Qfunc}_{\vec{\boldsymbol\lambda}, 2} (\vec\bsH'_2, +1)  $};
\node at (11.2, -5.5) {\small$\underline{\Qfunc}_{\vec{\boldsymbol\lambda}, 2} (\vec\bsH'_2, +1)  $};
\node at (11.2, -0.5) {\small$\overline{\Qfunc}_{\vec{\boldsymbol\lambda}, 2} (\vec\bsH'_2, -1)  $};
\node at (11.2, -1.5) {\small$\underline{\Qfunc}_{\vec{\boldsymbol\lambda}, 2} (\vec\bsH'_2, -1)  $};

\end{tikzpicture}
\caption{The stage-$2$ information $\vec{\bsH}_2 = (\vec{\bsH}_1, a_1 = + 1, R_1(+1) \mid \vec{\bsH}_1)$ and $\vec{\bsH}'_2 = (\vec{\bsH}_1, a_1 = -1, R_1(-1) \mid \vec{\bsH}_1)$. The superscript $\pi^\ast$ of stage-$1$ Q-functions represent their dependence on the IV-optimal stage-$2$ decision rule. The stage-$1$ interval $\big[\underline{\Qfunc}^{\pi^\ast}_{\vec{\boldsymbol\lambda}, 2} (\vec\bsH_2, +1), \overline{\Qfunc}^{\pi^\ast}_{\vec{\boldsymbol\lambda}, 2} (\vec\bsH_2, +1)\big]$ is the partial identification interval of the cumulative rewards of interest when we take $a_1 = +1$ and set $a_2$ to the optimal decision rule according to $\vec{\bsH}_2 = (\vec{\bsH}_1, a_1 = + 1, R_1(+1) \mid \vec{\bsH}_1)$}
    \label{fig: illustrate two stages}
\end{figure}

Figure \ref{fig: illustrate two stages} gives a graphical representation of the decision making process under our framework. At the second stage, given $\vec{\bsH}_2 = (\vec{\bsH}_1, a_1 = + 1, R_1(+1) \mid \vec{\bsH}_1)$ (or $\vec{\bsH}'_2 = (\vec{\bsH}_1, a_1 = -1, R_1(-1) \mid \vec{\bsH}_1)$) and $\lambda(\vec\bsH_2, +1) = \lambda(\vec\bsH_2, -1) = 1/2$ (corresponding to minimizing the maximum second stage risk; see Section \ref{subsec:alternative characterization} and Figure \ref{fig: illustrate stage k}), an IV-optimal decision is made based on comparing $0.5\cdot\big(\overline{\Qfunc}_{\vec{\boldsymbol\lambda}, 2} (\vec\bsH_2, +1) + \underline{\Qfunc}_{\vec{\boldsymbol\lambda}, 2} (\vec\bsH_2, +1)\big)$ with $0.5\cdot\big(\overline{\Qfunc}_{\vec{\boldsymbol\lambda}, 2} (\vec\bsH_2, -1) + \underline{\Qfunc}_{\vec{\boldsymbol\lambda}, 2} (\vec\bsH_2, -1)\big)$. Let $\pi^\ast_2$ denote the IV-optimal decision at the second stage and $V_2^{\pi^\ast}(\vec{\bsH}_2)$ the corresponding value. Importantly, $V_2^{\pi^\ast}(\vec{\bsH}_2)$ is some function of the first-stage reward $R_1(a_1)$ conditional on $\vec{\bsH}_1$.

At the first stage, the best-case and worst-case Q-functions $\overline{\Qfunc}_{\vec{\boldsymbol\lambda}, 1} (\vec\bsH_1, +1)$ and $\underline{\Qfunc}_{\vec{\boldsymbol\lambda}, 1} (\vec\bsH_1, +1)$ are estimating the upper and lower bounds of the expected cumulative rewards if we were to let $a_1 = +1$ and $a_2 = \pi_2^\ast(\vec{\bsH}_2)$. In other words, conditional on $\vec{\bsH}_1$, they are bounds on the expectation of the pseudo-outcome $R_1(+1) + V_2^{\pi^\ast}(\vec{\bsH}_2)$ or more explicitly $R_1(+1) + V_2^{\pi^\ast}(\vec{\bsH}_1, a_1 = +1, R_1(+1))$. Similarly, $\overline{\Qfunc}_{\vec{\boldsymbol\lambda}, 1} (\vec\bsH_1, -1)$ and $\underline{\Qfunc}_{\vec{\boldsymbol\lambda}, 1} (\vec\bsH_1, -1)$ are partial identification intervals of the pseudo-outcome $R_1(-1) + V_2^{\pi^\ast}(\vec{\bsH}_1, a_1 = -1, R_1(-1))$. Again, the first-stage decision is made based on comparing $\overline{\Qfunc}_{\vec{\boldsymbol\lambda}, 1} (\vec\bsH_1, \pm 1)$ and $\underline{\Qfunc}_{\vec{\boldsymbol\lambda}, 1} (\vec\bsH_1, \pm 1)$ for some choice of constants $\lambda(\vec{\bsH}_1, \pm 1)$.

In practice, we would follow Algorithm \ref{alg}, replace relevant quantities (first- and second-stage Q-functions and $V_2^{\pi^\ast}(\vec{\bsH}_2)$) with estimated values, and run a weighted classification routine to estimate the decision rule at each stage. To illustrate, we generated data ($n = 2,000$) according to the above DGP, estimate bounds using the Manski-Pepper bounds, and estimated a decision rule at each stage using a classification tree with $\lambda(\vec\bsH_2, \pm 1) = \lambda(\vec\bsH_1, \pm 1) = 1/2$. Figure \ref{fig: illustrate two-stage tree} plots the resulting IV-optimal DTR that minimizes the maximum risk at each stage.

